Universal Approximation for Log-concave Distributions using Well-conditioned Normalizing Flows

Normalizing flows are a widely used class of latent-variable generative models with a tractable likelihood. Affine-coupling (Dinh et al, 2014-16) models are a particularly common type of normalizing flows, for which the Jacobian of the latent-to-observable-variable transformation is triangular, allowing the likelihood to be computed in linear time. Despite the widespread usage of affine couplings, the special structure of the architecture makes understanding their representational power challenging. The question of universal approximation was only recently resolved by three parallel papers (Huang et al.,2020;Zhang et al.,2020;Koehler et al.,2020) -- who showed reasonably regular distributions can be approximated arbitrarily well using affine couplings -- albeit with networks with a nearly-singular Jacobian. As ill-conditioned Jacobians are an obstacle for likelihood-based training, the fundamental question remains: which distributions can be approximated using well-conditioned affine coupling flows? In this paper, we show that any log-concave distribution can be approximated using well-conditioned affine-coupling flows. In terms of proof techniques, we uncover and leverage deep connections between affine coupling architectures, underdamped Langevin dynamics (a stochastic differential equation often used to sample from Gibbs measures) and H\'enon maps (a structured dynamical system that appears in the study of symplectic diffeomorphisms). Our results also inform the practice of training affine couplings: we approximate a padded version of the input distribution with iid Gaussians -- a strategy which Koehler et al.(2020) empirically observed to result in better-conditioned flows, but had hitherto no theoretical grounding. Our proof can thus be seen as providing theoretical evidence for the benefits of Gaussian padding when training normalizing flows.

==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> derivative-bound.tex <==
%!TEX root=main.tex
\section{Derivative bound}

In this section we bound $\ln \rho_t(x)$.

To warm up, let's first consider overdamped Langevin. \hlnote{For underdamped Langevin, need more general form of Girsanov, compare to Brownian motion with momentum.}

We assume:
\begin{itemize}
    \item $\rh_0(x) = e^{-f_0(x)}$ satisfies $\ve{\nb f(x)}\le C_2\ve{x}$. \hlnote{For simplicity, let's actually consider $x_0\sim N(0,\si_0^2)$.}
    \item $f$ is twice-differentiable with $\ve{\nabla^2 f(x)}\le L_2$.
    \item $f(x)$ is $(m,b)$ dissipative:
    \begin{align*}
        \an{x,\nb f(x)} &\ge m\ve{x}^2-b.
    \end{align*}
\end{itemize}

Overdamped Langevin is given by the equation
\begin{align*}
    dx_t &= -\rc2\nb f(x_t) + \, dB_t.
\end{align*}
We aim to bound $\nb \ln \rh_T(x)$.
By Girsanov's Theorem, letting
\begin{align*}
    \La &= \exp\pa{\rc 2\int_0^T \nb f(x_s)^*\,dB_s - \rc 8 \int_0^T \ve{\nb f(x_s)}^2\,ds},
\end{align*}
we have that $x_t$ is Brownian motion under $\Q(A) = \E_\Pj(\La \one_A)$. 
Using $dB_s = dx_s + \rc 2 \nb f(x_s)$, 
\begin{align*}
    \La^{-1} &= \exp\pa{-\rc 2\int_0^T \nb f(x_s)^*\,dx_s
    - \rc 8 \int_0^T \ve{\nb f(x_s)}^2\,ds}.
\end{align*}
We derive the density function $\rh_t(z)$ by noting it is the function such that 
\begin{align*}
    \int_{A} \rh_t(z)\,dz &= \E_{x_t\sim \rh_t}[\one_A]
    = \frac{\E_{x\sim \W} [\La^{-1} \one_{x_t\in A}]}{\E_{\W}[\La^{-1}]}\\
    &= \frac{\E_{x_t\sim N(x_0,t), x_0\sim \rh_0} [\E_{x\sim \W}[\La^{-1}|x_t=x] \one_{x_t\in A}]}{\E_{\W}[\La^{-1}]}\\
    &= \int_A \rc{(2\pi (\si_0^2+t))^{d/2}} e^{-\fc{\ve{x}^2}{2(\si_0^2+t)}} \fc{\E_{x\sim \W}[\La^{-1}|x_t=x]}{\E_{\W}[\La^{-1}]}\,dx .
\end{align*}
%\hlnote{I think i'm missing a factor - probability that Brownian motion ends up at $z$?}
Thus
\begin{align}
    \rh_t(z) &= \rc{(2\pi (\si_0^2+t))^{d/2}} e^{-\fc{\ve{z}^2}{2(\si_0+t)}} \frac{\E_{x\sim \W}[\La^{-1}| x_t=z]}{\E_{\W}[\La^{-1}]}
    \label{e:rhot}
    %\\
    %\nb_z \ln \rh_t(z) &= 
    %- \fc{z}{\si_0^2+t}+ \nb_z \ln \E_{x\sim \W}[\La^{-1}| x_t=z]
\end{align}
where $\W$ denotes the Wiener process (started with initial distribution $\rh_0$). 
We now ``couple" paths arriving at $z$ and $z+y$ by translating each path by $y$. This will give an expression for $\rh_t(z+y)$ in terms of an expectation $\E_{x\sim \W}[\cdot |x_t=z]$. 
\begin{align*}
\int_A \rh_t(z+y)\,dz =
    \int_{A+y} \rh_t(z) \,dz &= \frac{\E_{x\sim \W}[\La^{-1} \one_{x_t\in A+y}]}{\E_{\W}[\La^{-1}]}
    \\
    &= \frac{\E_{x'=x-y\sim \W}\ba{
    \fc{\rh_0(x_0'+y)}{\rh_0(x_0')}
    \La^{-1}(x'+y) \one_{x_t'\in A}}}{\E_{\W}[\La^{-1}]}
\end{align*}
where we make a change of variable, defining the path $x'$ by $x_t' = x_t - y$, and note that if we draw $x'\sim \W$, then we have to reweight by $\fc{\rh_0(x_0)}{\rh_0(x_0')}$. This equals
\begin{align*}
    \int_{A} \rh_t(z+y)\,dz
    &= \int_{A} \rc{(2\pi (\si_0^2+t))^{d/2}} e^{-\fc{\ve{z'}^2}{2(\si_0^2+t)}}
    \fc{\E_{x'\sim \W}\ba{\fc{\rh_0(x_0'+y)}{\rh(x_0')}
    \La^{-1}(x'+y) | x_t'=z'}}{\E_{\W}[\La^{-1}]}\,dz' \\
\implies \rh_t(z+y)    &= \rc{(2\pi (\si_0^2+t))^{d/2}} e^{-\fc{\ve{z}^2}{2(\si_0^2+t)}}
    \fc{\E_{x\sim \W}\ba{\fc{\rh_0(x_0+y)}{\rh(x_0)}
    \La^{-1}(x+y) | x_t=z}}{\E_{\W}[\La^{-1}]} 
\end{align*}
Note that $y=0$ recovers~\eqref{e:rhot}.
% By a change-of-variable,
% \begin{align*}
%     \E_{x\sim \W}[\La^{-1}| x_t=z+y] &= 
%     \E_{x\sim \W}\ba{\fc{\rh_0(x_0+y)}{\rh_0(x_0)}\La^{-1}| x_t=z}
%     =\E_{x\sim \W}\ba{\exp\pa{f_0(x_0)-f_0(x_0+y)}\La^{-1}| x_t=z}
% \end{align*}
Therefore, 
\begin{align*}
    \nb_z \ln \rh_t(z) &=% - \fc{z}{\si_0^2+t}+
    \frac{\E_{x\sim \W}\ba{
    \pa{-\nb f_0(x_0) -\rc2 \int_0^T \nb^2f(x_s)\,dx_s -\rc 8 \int_0^T \nb^2 f(x_s)\nb f(x_s)\,ds}
    \La^{-1} | x_t = z
    }}{
    \E_{x\sim \W}\ba{
    \La^{-1} | x_t = z
    }
    }
\end{align*}
We want to show that on average (over Langevin paths ending up at $x_t=z$) that $x_s$ stays bounded. We use Girsanov's theorem to establish this by comparing with the Brownian bridge.
We show that for paths where $x_s$ stays bounded, the factor $\La^{-1}$ is bounded below, while for paths where $x_s$ is very large, the factor $\La^{-1}$ is very small. Thus the probability of $x_s$ being large can be bounded by the corresponding probability for the Brownian bridge.
%so that we can estimate the probability mass using the Brownian bridge, 

First, we rewrite $\La^{-1}$. Note that dissipativity and the Lipschitz bound on the derivative imply
\begin{align*}
    m\ve{x}- \fc{b}{\ve{x}} \le \ve{\nb f} \le L_2\pa{\ve{x}+\sfc bm}
\end{align*}
By dissipativity, $\nb f(x_s)$ has large projection onto $x_s$:
\begin{align*}
    \an{\fc{\nb f(x_s)}{\ve{x_s}}, \fc{x_s}{\ve{x_s}}} &\ge m - \fc{b}{\ve{x_s}^2}.
\end{align*}
Thus we can bound the component that is perpendicular to $x_s$:
\begin{align*}
    \ve{\nb f(x_s) - \an{\fc{\nb f(x_s)}{\ve{x_s}}, \fc{x_s}{\ve{x_s}}} x_s} &\le \pa{1-\fc{m-\fc{b}{\ve{x_s}^2}}{L_2\pa{1+\fc{\sqrt{b/m}}{\ve{x_s}^2}}}}\ve{\nb f(x_s)}=:c_{\ve{x_s}}\ve{\nb f(x_s)}.
\end{align*}
Let
\begin{align*}
    \nb^{\parallel} f(x_s) &= \an{\fc{\nb f(x_s)}{\ve{x_s}}, \fc{x_s}{\ve{x_s}}}  x_s\\
    \nb^{\perp} f(x_s) &=\nb f(x_s) -  \nb^{\parallel} f(x_s) .
\end{align*}
Thus
\begin{align*}
    -\rc 2 \int \pa{\nb^{\parallel}f(x_s) + \nb^\perp f(x_s)}\,dx_s
    &\le \int -\rc 2 (m-\cdots) x_s\,dx_s
    + \rc 2\int  c_{\ve{x_s}} \ve{\nb f(x_s)}\,dx_s.
\end{align*}
TODO: $\int x_s\,dx_s$ is positive (quadratic variation of Brownian motion), look at small $x_s$ separately.  use AM-GM on second term. this can increase the variance of the Brownian motion. If $x_s$ is large $=L$ then by Brownian bridge this contributes $\exp(-L^2/2...)$ which swamps out whatever weight $\La^{-1}$ has.

==> discard.tex <==
\section{discarded euler discretization}
We consider a more general ODE than the specific one in \eqref{eqn:affine_coupling_ode}, of the form
\begin{equation}
\label{eqn:general_euler}
    \frac{d}{dt}(y(t)) = f(y(t), t)
\end{equation}
and consider discretizing this ODE into steps of size $\eta$, as follows:
\begin{align*}
    Y_{i+1} = Y_i + \eta f(Y_i, \eta i)
\end{align*}
Further, let
\begin{align*}
    y_i &= y(\eta i)
\end{align*}
Here, $Y_0 = y_0 = y(0)$. From \cite{??}, we know that 
\begin{align*}
    \sup_{y_0 \in \mathcal{C}} \norm{Y_i - y_i} =
    \fc{M\eta}{2L} [e^{L\eta i}-1]=
    O(\eta)
\end{align*}
\fixme{where $M=\max_{0\le t\le T} |y''(t)|$ and $f$ is $L$-Lipschitz in $y$.}
Now, to show closeness in $C^1$ topology over a compact set $\mathcal{C}$, we need to bound $\sup_{y_0 \in \mathcal{C}} \norm{DY_i - Dy_i}$.

To prove this, we express the Euler discretization as composition of functions. Let $S_i$ denote the map $y \mapsto y + \eta f(y,\eta i)$. Then $Y_i$ is given as $S_{i-1} \circ \cdots \circ S_{0}(Y_0)$. Let $A_i$ denote the flow map $T_{\eta i, \eta (i+1)}$ for \eqref{eqn:general_euler}. Then $y_i = A_{i-1} \circ \cdots \circ A_0 (y_0)$.
Observe that by Taylor's theorem,
\[ A_i(y) = y + \eta f(y,\eta i) + \frac{\eta^2}{2} \ddot{y}(t^*) \]
for some $t^* \in [\eta i, \eta(i+1)]$. 
Note that by the total derivative rule, we have
\[ \ddot{y}(t^*) = D_t f(y(t^*),t^*) + D_y f(y(t^*),t^*) \cdot f(y(t^*),t^*) \]
Therefore,
\[ \norm{A_i - S_i}_\infty \le \frac{\eta^2}{2} \brac{\norm{D_t f} + \norm{D_yf} \norm{f}} \]
Note that since $\mathcal{C}$ is compact, and $f$ is smooth in $y,t$, all these terms are bounded over $\mathcal{C}$, which gives us that $\norm{A_i - S_i} = O(\eta^2)$.

Similarly,
\[ D_y S_i = \id + \eta D_y f(y, \eta i) \]
on the other hand, using \Cref{l:ode_derivative},
\[ D_y A_i = \id + \eta D_y f(y,\eta i) + \frac{\eta^2}{2} \left.\frac{d}{dt}\right\vert_{t^*} \brac[\Big]{D_y f(y(t),t) D_y(T_{\eta i, t})} \]
for some $t^* \in [0,\eta]$ where $y(t) = T_{\eta i, t}(y)$. Now, we bound the last term in the RHS above.
\begin{align*}
     & \frac{d}{dt} \brac[\Big]{D_y f(y(t),t) D_y(T_{\eta i, t})}\\
     = & \frac{d}{dt} \brac[\Big]{D_y f(y(t), t)} D_y(T_{\eta i,t}) + D_y f(y(t),t) \frac{d}{dt} \brac[\Big]{D_y(T_{\eta i, t})}\\
     = & \brac{\frac{d}{dt} D_y f (y(t),t) + D^2_y f(y(t),t)} D_y(T_{\eta i, t}) + D_y f(y(t),t) D_y\brac{\frac{d}{dt} y(t)} \\
     = & D_y \brac[\Big]{D_t f(y,t) + D_y f(y,t) \cdot f(y,t)} \cdot D_y(T_{\eta i, t}) + D_y f(y,t) \cdot D_y(f(y,t))\\
     = & \brac[\Big]{D_y D_t f(y,t) + D^2_y f(y,t) + Df(y,t)^2} \cdot D_y(T_{\eta i, t}) + D_y(f(y,t))^2 \\
     = & 
\end{align*}

\begin{align}
    \norm{Y_{n+1} - y_{n+1}}_{C^1} 
    & = \norm{A_n \circ \cdots \circ A_0 - S_n \circ \cdots \circ S_0}_{C^1}\\
        & \le \norm{A_n \circ \cdots \circ A_1 \circ A_0 - A_n \circ \cdots \circ A_1 \circ S_0}_{C^1} \\
        & + \norm{A_n \circ \cdots \circ A_1 \circ S_0 - S_n \circ \cdots \circ S_1 \circ S_0}_{C^1} \tag{by triangle inequality}\\
        & \le \norm{A_n \circ \cdots \circ A_1 \circ A_0 - A_n \circ \cdots \circ A_1 \circ S_0}_\infty\\
        & + \norm{D(A_n \circ \cdots \circ A_1)\vert_{A_0(x)} \circ DA_0\vert_x - D(A_n \circ \cdots \circ A_1)\vert_{S_0(x)} \circ DS_0\vert_x}_\infty \tag{by chain rule}\\
        & + \norm{A_n \circ \cdots \circ A_1 \circ S_0 - S_n \circ \cdots \circ S_1 \circ S_0}_{C^1}  \\
        & \le \norm{D(A_n \circ \cdots \circ A_1)} \norm{A_0 - S_0}_\infty\\
        & + \norm{D(A_n \circ \cdots \circ A_1)\vert_{A_0(x)} \circ DA_0\vert_x - D(A_n \circ \cdots \circ A_1)\vert_{S_0(x)} \circ DA_0\vert_x}_\infty\\
        & + \norm{D(A_n \circ \cdots \circ A_1)\vert_{S_0(x)} \circ DA_0\vert_x - D(A_n \circ \cdots \circ A_1)\vert_{S_0(x)} \circ DS_0\vert_x}_\infty\\
        & + \norm{A_n \circ \cdots \circ A_1 \circ S_0 - S_n \circ \cdots \circ S_1 \circ S_0}_{C^1}  \\
        & \le \norm{D(A_n \circ \cdots \circ A_1)} \norm{A_0 - S_0}_\infty\\
        & + \norm{D(A_n \circ \cdots \circ A_1)\vert_{A_0(x)} - D(A_n \circ \cdots \circ A_1)\vert_{S_0(x)}} \norm{DA_0}  \\
        & + \norm{D(A_n \circ \cdots \circ A_1)} \norm{DA_0\vert_x - DS_0\vert_x}\\
        & + \norm{A_n \circ \cdots \circ A_1 - S_n \circ \cdots \circ S_1}_{C^1}\\
        & \le \norm{D(A_n \circ \cdots \circ A_1)} \norm{A_0 - S_0}_\infty\\
        & + \norm{D^2(A_n \circ \cdots \circ A_1)} \norm{A_0 - S_0} \norm{DA_0}  \\
        & + \norm{D(A_n \circ \cdots \circ A_1)} \norm{DA_0 - DS_0}\\
        & + \norm{A_n \circ \cdots \circ A_1 - S_n \circ \cdots \circ S_1}_{C^1}\\
        & \le \kappa O(\eta^2) + \kappa \kappa_2 O(\eta^2) + \kappa O(\eta^2) + \norm{A_n \circ \cdots \circ A_1 - S_n \circ \cdots \circ S_1}_{C^1}\\
        & \le n O(\eta^2) \tag{by induction}
        % & + \norm{D(DA_n \circ \cdots \circ 
        % & \le \sum_{i=1}^{n+1} \norm{D T_{i\tau, \timethree -i \tau}} \norm{S'_{i-1} - A_{i-1}}_{C^1}
        % \tag{by induction}
        % \\
        % & \le (n+1)\cdot (O(\eta) + O(\tau^2)) = \fc{\timethree}{\tau} \cdot {(O(\eta) + O(\tau^2))} = O\left(\frac{\eta}{\tau}\right) + O(\tau)
\end{align}
Therefore, total error in $C_1$ topology over $\mathcal{C}$ is $O(n\eta^2)$ where $n$ is the number of steps.


==> gradient_flow.tex <==
%!TEX root=main.tex
\section{Gradient flow for distributions}
Suppose we have a target distribution $\mathbf{p}^*(x)$ that we want to approximate. \cite{ma2019mcmc} describe a momentum method to find $\mathbf{p}^*$ from some starting distribution $\mathbf{p}$ using a variant of accelerated gradient descent. For this, a momentum variable $v$ is added so that $\mathbf{p}^*(x,v) \propto \exp(-U(x) - \frac{\xi}{2} \norm{v}_2^2)$, for some function $U$. Then the gradient flow converging to $\mathbf{p}^*$ is given by equations $(6), (7)$ from \cite{ma2019mcmc} as
\begin{align}
\label{eq:gradient_flow}
    \begin{bmatrix} \frac{dx}{dt} \\ \frac{dv}{dt} \end{bmatrix}
    & = - \begin{bmatrix} 0 & -I \\ I & \gamma I \end{bmatrix} \begin{bmatrix} \nabla_x \frac{\delta \KL(\mathbf{p}_t \Vert \mathbf{p}^*)}{\delta \mathbf{p}_t} \\ \nabla_v \frac{\delta \KL(\mathbf{p}_t \Vert \mathbf{p}^*)}{\delta \mathbf{p}_t} \end{bmatrix}   
\end{align}
Further, they give a guarantee that the Lyapunov functional $\mathcal{L}$ given by 
\[ \mathcal{L}[\mathbf{p}_t] = \KL(\mathbf{p}_t \Vert \mathbf{p}^*) + \mathbb{E}_{\mathbf{p}_t} \left[ \left\langle \nabla_x \frac{\delta \KL(\mathbf{p}_t \Vert \mathbf{p}^*)}{\delta \mathbf{p}_t}, S \nabla_x \frac{\delta \KL(\mathbf{p}_t \Vert \mathbf{p}^*)}{\delta \mathbf{p}_t} \right\rangle \right] \], where $S$ is pd matrix given by
\[ S = \frac{1}{L_G} \begin{bmatrix} \frac{1}{4} I_{d \times d} & \frac{1}{2} I_{d \times d}  \\ \frac{1}{2} I_{d \times d}  & 2 I_{d \times d} \end{bmatrix}  \]
satisfies that 
\[ \frac{d}{dt} \mathcal{L}[\mathbf{p}_t] \le - \frac{\rho}{10} \mathcal{L}[\mathbf{p}_t] \]
which gives us linear rate of convergence in $\KL$ metric. Thus, running this gradient flow for time $T > - \frac{10 \log \epsilon}{\rho}$ will get us to a distribution $\mathbf{p}_T$ such that $\KL( \mathbf{p}_T \Vert \mathbf{p}^*) \le \epsilon$.

Here $L_G$ is the lipschitz constant of $\nabla U$ and $\rho$ is the log-sobolev parameter for $\mathbf{p}^*$.


==> langevin_preliminaries.tex <==
\section{Underdamped Langevin Dynamics}
\label{sec:langevin_preliminaries}

In this section, we describe the specifics of running underdamped Langevin dynamics to derive a sample from a target distribution, and the existing results on their convergence. We tailor the SDE's involved to our particular problem setting; for a more extensive review on Langevin dynamics, we refer the reader to \cite[Chapter 6]{pavliotis2014stochastic}. The target distribution that we are concerned with here is the standard Gaussian in $\R^{2d}$, a choice which we will justify in the subsequent section.

The underdamped Langevin dynamics with stationary distribution $p^*(x,v) \propto e^{-\frac{1}{2}(\norm{x}^2 + \norm{v}^2)}$ is given by the following SDE's,
\begin{align}\label{e:m-uld-1}
    dx_t &= -v_t\\
    dv_t &= -\ga v_t - x_t + \sqrt{2}\, dB_t.    
    \label{e:m-uld-2}
\end{align}

We can convert this SDE to an equivalent ODE below (with time-dependent coefficients), as given by (\cite{ma2019mcmc} equations $(6),(7)$). It is easy to check that the differential equations below give the same distributions over time. %by writing their Fokker-Planck formats.
\begin{align}
\label{eq:gradient_flow}
    \begin{pmatrix} \frac{dx}{dt} \\ \frac{dv}{dt} \end{pmatrix}
    & = - \begin{pmatrix} 0 & -I \\ I & \gamma I \end{pmatrix} \begin{pmatrix} \nabla_x \frac{\delta \KL(p_t \Vert p^*)}{\delta p_t} \\ \nabla_v \frac{\delta \KL(p_t \Vert p^*)}{\delta p_t} \end{pmatrix}   
\end{align}
where $p_0 = p(x,v) \propto e^{-U(x)-\frac{\|v\|^2}{2}}$ is the initial distribution. This simplifies to
\begin{align}\label{e:m-uld-3}
    \ddd t\coltwo{x_t}{v_t} 
    &=
    \matt{O}{I_d}{-I_d}{-\ga I_d} (\nb \ln p_t - \nb \ln p^*)
\end{align}
Running underdamped Langevin \eqref{e:m-uld-3} as defined above to convergence yields a sample from the target distribution $p^*$. \cite{ma2019mcmc} give a rate of convergence using Lyapunov function $\mathcal{L}$, \hlnote{I thought that we only have convergence for $\mathcal L = \KL+\cdots$, not $\KL$ directly?}
\[ \mathcal{L}[p_t] = \KL(p_t \Vert p^*) + \mathbb{E}_{p_t} \left[ \left\langle \nabla \frac{\delta \KL(p_t \Vert p^*)}{\delta p_t}, S \nabla \frac{\delta \KL(p_t \Vert p^*)}{\delta p_t} \right\rangle \right] \], where $S$ is positive definite matrix given by
\[ S = \frac{1}{\kappa} \begin{bmatrix} \frac{1}{4} I_{d \times d} & \frac{1}{2} I_{d \times d}  \\ \frac{1}{2} I_{d \times d}  & 2 I_{d \times d} \end{bmatrix}  \]
satisfies that 
\begin{equation}
\label{e:L-ma-mcmc}
    \frac{d}{dt} \mathcal{L}[p_t] \le - \frac{\rho}{10} \mathcal{L}[p_t] 
\end{equation}
whenever $p^*$ satisfies a log-Sobolev inequality with constant $\rho$. Since we are going to use the underdamped Langevin dynamics with $p^* = \mathcal{N}(0,\id)$, $\rho = 1$ suffices. 

Since $\mathcal{L}[p_t] > \KL(p_t \Vert p^*)$, because $S$ is positive definite, this gives us linear rate of convergence in $\KL$ metric. Thus, running this gradient flow for time $T > - 10 \log \epsilon + \log \mathcal{L}[p_0]$ will get us to a distribution $p_T$ such that $\KL( p_T \Vert p^*) \le \epsilon$. In the following, we show that the term $\mathcal{L}[p_0]$ is finite:

\Snote{This part probably belongs to proof sketch}
\begin{align*}
    \mathcal{L}[p_0] 
    & = \mathbb{E}_{p_0} \left[ -U(x) + \frac{\norm{x}^2}{2} + \left\langle \nabla \left(-U(x) + \frac{\norm{x}^2}{2} \right), S \nabla \left( -U(x) + \frac{\norm{x}^2}{2} \right) \right\rangle \right]\\
    & = \mathbb{E}_{p_0} \left[ -U(x) + \frac{\norm{x}^2}{2} + \frac{1}{4 \kappa} \norm{- \nabla U(x) + x}^2  \right] \\
    &\le \mathbb{E}_{p_0} \left[ -U(x) + \frac{\norm{x}^2}{2} + \frac{1}{4 \kappa} (\|\nabla U(x)\|^2 + \|x\|^2 + 2\|\nabla U(x)\|\|x\|)  \right] \\
    &\le \mathbb{E}_{p_0} \left[ -U(x_0) - \frac{\|x-x_0\|^2}{2} + \frac{\norm{x}^2}{2} + \frac{1}{4 \kappa} (\kappa^2\|x-x_0\|^2 + \|x\|^2 + 2\kappa\|x-x_0\|\|x\|)  \right] \\
    &\le \mathbb{E}_{p_0} \left[ -U(x_0) - \frac{\|x-x_0\|^2}{2} + \frac{\norm{x}^2}{2} + \frac{1}{4 \kappa} (\kappa^2\|x-x_0\|^2 + \|x\|^2 + 2\kappa\|x\|^2+2\kappa\|x_0\|\|x\|)  \right]
\end{align*}
where $x_0$ is the mode of $p_0$ above. Here, we notice that each term in the computation of the expectation above is either of the form $\int \|x\|^2 e^{-U(x)}\;dx$ or $\int \|x\|e^{-U(x)}\;dx$. Since these integrals are finite ($p_0$ is log-concave), we have that $\mathcal{L}[p_0] < \infty$.
\Snote{Do we need to bound $\mathcal{L}[p_0]$ in terms of $\KL(p_0 \Vert p^*)$? -- $\KL$ is the original benchmark}


==> overdamped-condition.tex <==
We bound the condition number of the transport map induced by Langevin. First consider overdamped Langevin.

\begin{lemma}\label{l:convolve-lc}
Suppose that $p$ is a probability density function on $\R^d$ such that $-\ln p$ is $\al$-convex and $\be$-smooth. 
Let $q\propto e^{-\rc2 \ga\ve{x}^2}$ be the pdf of $N(0,\si^2 I_d)$, where $\si^2 = \rc{\ga}$. Then 
$-\ln (p*q)$ is $\fc{\al\ga}{\al+\ga}$-convex and $\fc{\be \ga}{\be + \ga}$-smooth.
\end{lemma}
\begin{proof}
We have $(p*q)(x) = \int_{\R^d} p(t)q(x-t)\,dt$, so 
\begin{align*}
    \nb^2 [\ln ((p*q)(x))] &= 
    \fc{\int_{\R^d} p(t) \nb^2 q(x-t)\,dt}{\int_{\R^d} p(t)  q(x-t)\,dt}
    - 
    \pf{\int_{\R^d} p(t) \nb q(x-t)\,dt}{\int_{\R^d} p(t)  q(x-t)\,dt}
    \pf{\int_{\R^d} p(t) \nb q(x-t)\,dt}{\int_{\R^d} p(t)  q(x-t)\,dt}^\top\\
    &= 
    \ga^2 \pf{\int_{\R^d} (x-t) p(t) q(x-t)\,dt}{\int_{\R^d} p(t)  q(x-t)\,dt}
    \pf{\int_{\R^d} (x-t)^\top p(t) q(x-t)\,dt}{\int_{\R^d} p(t)  q(x-t)\,dt} \\
    &\quad - 
    \fc{\int_{\R^d} (\ga^2 (x-t)(x-t)^\top - \ga I_d) p(t) q(x-t)\,dt}{\int_{\R^d} p(t)  q(x-t)\,dt}
\end{align*}
Let $\mu_x$ denote the distribution with density function $\rh(t) \propto p(t)q(x-t)$. Then this equals
\begin{align*}
    \ga^2[\E_{\mu_x} (t-x)][\E_{\mu_x} (t-x)^\top]
    - [\E_{\mu_x} (t-x)(t-x)^\top] + \ga I_d
    &= 
    -\ga^2\E_{\mu_x} [(t-\E t)(t-\E t)^\top] + \ga I_d.
\end{align*}
Note the first term is the covariance of $t$.
Note that $\mu_x$ is $(\al+\ga)$-log-concave. Thus by Harg\'e's Theorem~\ref{thm:harge}, for any unit vector $v$,
\begin{align*}
    v^\top \nb^2 [\ln ((p*q)(x))]v &\ge-\ga^2 \E_{t\sim N(0,\rc{\al+\ga})}\an{t,v}^2 +\ga \ge 
    -\ga^2\rc{\al+\ga} + \ga = \fc{\al \ga}{\al+\ga}.
\end{align*}
\fixme{By the reverse direction of Harg\'e} \hlnote{I can't find the statement of this in the literature, but I think it should hold. We only need this for a quadratic.}
\begin{align*}
    v^\top \nb^2 [\ln ((p*q)(x))]v &\le -\ga^2\E_{t\sim N(0,\rc{\be+\ga})}\an{t,v}^2+\ga \le 
    -\ga^2\rc{\be+\ga} + \ga = \fc{\be \ga}{\be+\ga}.
\end{align*}
\end{proof}

\begin{theorem}[{Harg\'e, \cite{harge2004convex}}]\label{thm:harge}
Suppose the $d$-dimensional gaussian $N(0,\Si)$ has density $\ga$. Let $p=h\cdot \ga$ be a probability density, where $h$ is log-concave. Let $g:\R^d\to \R$ be convex. Then
\begin{align}
\int_{\R^d} g(x-\E_p x)p(x)\,dx &\le \int_{\R^d} g(x)\ga(x)\,dx.
\end{align}
\end{theorem}

% \hlnote{I can't find the reverse direction of Harg\'e's inequality in the literature, but we can prove the version we need.}
% \begin{lemma}[Reverse of Harg\'e's inequality for quadratic]
% Suppose the $d$-dimensional gaussian $N(0,\Si)$ has density $\ga$. Let $p$ be a probability density with $p\cdot h=\ga$, where $h$ is log-concave. Let $g:\R^d\to \R$ be convex. Then
% \begin{align}
% \int_{\R^d} g(x-\E_p x)p(x)\,dx &\ge \int_{\R^d} g(x)\ga(x)\,dx.
% \end{align}
% \end{lemma}
The following tells us that for the Ornstein-Uhlenbeck process initialized on a log-concave distribution, the largest and smallest singular values of $-\nb^2 \ln p_t$ decay logistically towards 1.
\begin{lemma}\label{l:hess-bd}
Consider the Ornstein-Uhlenbeck process (overdamped Langevin with stationary measure $p(x)\propto e^{-f(x)}$, where $f(x) = -\rc 2\ve{x}^2$). 
Suppose that the initial distribution $p_0$ is such that $-\ln p_0$ is $\rc{\ka}$-strongly convex and 1-smooth. Then $-\ln p_t$ is $\rc{1+(\ka-1)e^{-2t}}$-strongly convex and 1-smooth.
\end{lemma}
\begin{proof}
\hlnote{TODO: Justify approximation using discretization.}
Consider taking a step of size $\eta$:
\begin{align*}
    \td x_{t+\eta}' &= \td x_t -\eta \nb f(\td x_t) = (1-\eta) \td x_t \\
    \td x_{t+\eta} &= \td x_{t+\eta}' + \xi, \quad \xi\in N(0,2\eta I_d).
\end{align*}
From this, the approximate distributions satisfy $\td p_{t+\eta} = \td p_t\pa{\rc{1-\eta}\cdot} * \ph_{2\eta I_d}$ where $\ph_\Si$ denotes the pdf of the gaussian $N(0,\Si)$. If $-\ln \td p_t$ is $\td \al_t$-convex and $\td \be_t$-smooth, then $\td p_t(\rc{1-\eta}x)$ is $\fc{\td \al_t}{(1-\eta)^2}$-convex and $\fc{\td \be_t}{(1-\eta)^2}$-smooth, so by Lemma~\ref{l:convolve-lc}, $-\ln \td p_{t+\eta}$ has strong convexity constant
\begin{align*}
    \fc{\fc{\td \al_t}{(1-\eta)^2} \rc{2\eta} }{\fc{\td \al_t}{(1-\eta)^2} + \rc{2\eta}} &=\td  \al_t - 2\eta \td \al_t (\td \al_t-1) + O(\eta^2)
\end{align*}
and smoothness constant
\begin{align*}
    \fc{\fc{\td \be_t}{(1-\eta)^2} \rc{2\eta} }{\fc{\td \be_t}{(1-\eta)^2} + \rc{2\eta}} &= \td \be_t - 2\eta \td \be_t (\td \be_t-1) + O(\eta^2)
\end{align*}
Taking $\eta\to 0$, we we derive the following bounds for the convexity and smoothness of $-\ln p_t$:
\begin{align*}
    \al_0 &= \rc{\ka} &
    \ddd t\al_t &= -2\al_t(\al_t-1) & \al_t &= \rc{1+(\ka-1)e^{-2t}}\\
    \be_0 &=1 &
    \ddd t \be_t &= -2\be_t(\be_t-1) & \be_t &= 1.
\end{align*}
\end{proof}
We use the following form of the Langevin equation (see~\cite[(31)]{taghvaei2019accelerated})
\begin{align}\label{e:lgv-flow}
    dx_t &= -\nb f(x_t)\,dt - \nb \ln p_t(x_t).
\end{align}
\begin{theorem}
Suppose that the initial distribution $p_0$ is such that $-\ln p_0$ is $\rc{\ka}$-strongly convex and 1-smooth. 
Let $T_t$ denote the transport map from time 0 to time $t$ induced by overdamped Langevin~\eqref{e:lgv-flow}. Then for any $x_0$ and unit vector $v$, the directional derivative of $T_t$ at $x_0$ in direction $v$ satisfies
\begin{align*}
    %\rc{e^{1/2}\min\{1,\sqrt{\ka-1}\}}
    \rc{\sqrt\ka} \le 
    \ve{D_v T_t(x_0)} \le 1
    %\sqrt\ka.
    %e^{1/2}\min\{1,\sqrt{\ka-1}\}.
\end{align*}
Thus the condition number of $T_t$ is bounded by $\sqrt\ka$. %$e\min\{1,\ka-1\}$.
\end{theorem}
\begin{proof}
We have that $T_t(x_0)=x_t$ where $x_t$ solves the equation
\begin{align*}
    x_t&=\int_0^t \nb (-f(x_s) +\ln p_s(x_s))\,ds.
\end{align*}
Then by the chain rule,
\begin{align*}
    %x_t &= \int_0^t \nb (-f(x_s)+\ln p_s(x_s))\,ds\\
    D_v T_t(x_0) &=\int_0^t \nb^2 (-f(x_s) + \ln  p_s(x_s)) D_vT_s(x_0)\,ds.
\end{align*}
Now by Lemma~\ref{l:hess-bd}, %\hlnote{Being more careful here we can probably say that actually this doesn't increase, and get $\sqrt{\ka}$ at the end}
\begin{align*}
    \ve{\nb^2 (-f(x_s)+\ln p_s(x_s))v} &\in \ba{0, 1-\rc{1+(\ka-1)e^{-2s}}}\cdot \ve{v}.
\end{align*}
Hence
\begin{align*}
    \ddd t \ve{D_vT_t(x_0)} &\ge-\pa{1-\rc{1+(\ka-1)e^{-2s}}} \ve{D_vT_t(x_0)}
    = -\pa{\fc{(\ka-1)e^{-2s}}{1+(\ka-1)e^{-2s}}} \ve{D_vT_t(x_0)}
\end{align*}
Moreover, because $\nb^2 (-f(x_s)+\ln p_s(x_s))v$ is negative definite by Lemma~\ref{l:hess-bd}, 
\begin{align*}
    \ddd t \ve{D_vT_t(x_0)} &\le 0.
\end{align*}
For unit vector $v$, $\ve{D_vT_0(x_0)}=\ve{v}=1$, so by Gronwall's inequality,
\begin{align*}
0\ge 
    %\ab{
    \ln \ve{D_v T_t(x_0)}
    %}
    &\ge - \int_0^t \fc{(\ka-1)e^{-2s}}{1+(\ka-1)e^{-2s}}\,ds\\
    %1-\rc{1+(\ka-1)e^{-2s}}\,ds.
    &= -\ba{-\rc 2 \ln (1+(\ka-1) e^{-2t})}_0^t \ge -\rc 2 \ln \ka.
\end{align*}
% For $s\le \rc 2\ln \prc{\ka-1}$, bound the integrand trivially by 1. For $s>\rc 2\ln \prc{\ka-1}$, we use the bound
% \begin{align*}
%     1-\rc{1+(\ka-1)e^{-2s}} &\le \rc 2 e^{-\pa{s-\rc 2 \ln \prc{\ka-1}}}.
% \end{align*}
% Thus letting $\ln_+ x = \max\{0,\ln x\}$
% \begin{align*}
%     \ab{
%     \ln \ve{D_v T_t(x_0)}
%     } &\le \rc2 \ln_+ \prc{\ka-1} + \int_0^\iy \rc 2 e^{-s}\,ds
%     = \rc2 \ln_+ \prc{\ka-1} +\rc2
% \end{align*}
The conclusion then follows.
\end{proof}

==> preliminaries.tex <==
\section{Preliminaries} 

Our techniques leverage tools from stochastic differential equations and dynamical systems. We briefly survey the relevant results. 

\subsection{Langevin Dynamics} 
\label{sec:langevin_dynamics}
Broadly, Langevin diffusions are families of stochastic differential equations (SDEs) which are most frequently used as algorithmic tools for sampling from distributions specified up to a constant of proportionality. They have also recently received a lot of attention as tools for designing generative models \citep{song2019generative, song2020score}. 

In this paper, we will only make use of \emph{underdamped Langevin dynamics}, a momentum-like analogue of the more familiar \emph{overdamped Langevin dynamics}, defined below. Our construction will involve simulating underdamped Langevin dynamics using affine coupling blocks.

\begin{definition}[Underdamped Langevin Dynamics] \emph{Underdamped Langevin dynamics} with potential $U$ and parameters $\ze$, $\ga$ is the pair of SDEs
\begin{align}\label{e:m-uld}
\begin{cases}
    dx_t &= -\zeta v_t dt\\
    dv_t &= -\ga \zeta v_t dt- \nabla U(x_t) dt + \sqrt{2 \gamma}\, dB_t.    
    \end{cases}
\end{align}
The stationary distribution of the SDEs (limiting distribution as $t \to \infty$) is given by $p^*(x,v) \propto e^{-U(x) - \fc{\zeta}2 \norm{v}^2}$.
\end{definition}

The variable $v_t$ can be viewed as a ``velocity'' variable and $x_t$ as a ``position'' variable -- in that sense, the above SDE is an analogue to momentum methods in optimization. 

The convergence of \eqref{e:m-uld} can be bounded when the distribution $p(x) \propto \exp(-U(x))$ satisfies an analytic condition, namely has a bounded \emph{log-Sobolev} constant. For completeness, the definition of a log-Sobolev constant is stated in \Cref{s:log_sobolev_inequalities}, though we will only need the following fact: 
\begin{fact}[\cite{bakry1985diffusions,bakry2013analysis}] Let the distributions $p(x) \propto \exp(-U(x))$ be such that $U(x) \succeq \lambda I$. Then, $p$ has log-Sobolev constant bounded by $\lambda$. 
\end{fact} 

The convergence time of underdamped Langevin dynamics was characterized in \cite{ma2019mcmc}: 

\begin{theorem}[\cite{ma2019mcmc}] 
\label{thm:L-ma_mcmc}
Let $p^*(x) \propto \exp(-U(x))$ have a log-Sobolev constant bounded by $\rho$. 
Furthermore, for a distribution $p: \R^d \to \R^{+}$, let %\anote{say somewhere $p^*$ will denote stationary}

\[ \mathcal{L}[p] := \KL(p \Vert p^*) + \mathbb{E}_{p} \left[ \left\langle \nabla \frac{\delta \KL(p \Vert p^*)}{\delta p}, S \nabla \frac{\delta \KL(p \Vert p^*)}{\delta p} \right\rangle \right], \] where $S$ is a positive definite matrix given by
$S = \frac{1}{\kappa} \begin{bmatrix} \frac{1}{4} I_{d \times d} & \frac{1}{2} I_{d \times d}  \\ \frac{1}{2} I_{d \times d}  & 2 I_{d \times d} \end{bmatrix}$. 
If $p_t$ is the distribution of $(x_t, v_t)$ which evolve according to \eqref{e:m-uld}, we have 
\begin{equation}
\label{e:L-ma-mcmc}
    \frac{d}{dt} \mathcal{L}[p_t] \le - \frac{\rho}{10} \mathcal{L}[p_t] 
\end{equation}
whenever $p^*$ satisfies a log-Sobolev inequality with constant $\rho$.
\end{theorem}

We note that the above theorem uses a non-standard Lyapunov function ($\mathcal{L}$), which combines KL divergence with an extra term, since the generator of underdamped Langevin is not self-adjoint -- this makes analyzing the drop in $KL$ divergence difficult. As $\mathcal{L}$ is clearly an upper bound on $KL(p || p^*)$, so it suffices to show $\mathcal L$ decreases rapidly. 

We will also need a less-well-known \emph{deterministic} form of the updates which is equivalent to \eqref{e:m-uld}. Precisely, we convert \eqref{e:m-uld} an equivalent ODE (with time-dependent coefficients). The proof of this fact (via a straightforward comparison of the Fokker-Planck equation) can be found in \cite{ma2019mcmc}. 
\begin{theorem}
Let $p_t(x_t, v_t)$ be the probability distribution of running \eqref{e:m-uld} for time $t$. If started from $(x_0, v_0) \sim p_0$, the probability distribution of the solution $(x_t, v_t)$ to the ODEs 
\begin{align}\label{e:m-uld-3-0}
    \ddd t\coltwo{x_t}{v_t} 
    &=
    \matt{O}{I_d}{-I_d}{-\ga I_d} (\nb \ln p_t - \nb \ln p^*)
\end{align}
is also $p_t(x_t, v_t)$.
\end{theorem}


\subsection{Dynamical systems and Henon maps} 

We also build on work from dynamical systems, more precisely, a family of maps called \emph{H\'enon-like maps} \citep{henon1976two}.
\begin{definition}[\citep{turaev2002polynomial}]
A pair of ODEs forms a \emph{H\'enon-like map} if it has the form
\begin{equation}
\label{eqn:ode_henon}
\begin{cases}  
\frac{dx}{dt} = v \\ 
\frac{dv}{dt} = -x + \nabla J(x)
\end{cases}
\end{equation}
for a smooth function $J: \R^d \to \R$.
\end{definition}
This special family of ODEs is a continuous-time generalization of a classical discrete dynamical system of the same name \cite{henon1976two}. The property that is useful for us is that the Euler discretization of this map can be written as a sequence of affine coupling blocks.

In \cite{turaev2002polynomial}, it was proven that these ODEs are \emph{universal approximators} in some sense. Namely, the iterations of this ODE can approximate any \emph{symplectic diffeomorphism}: a continuous map which preserves volumes (i.e. the Jacobian of the map is 1). These kinds of diffeomorphisms have their genesis in Hamiltonian formulations of classical mechanics \citep{abraham2008foundations}. 

At first blush, symplectic diffeomorphisms and underdamped Langevin seem to have nothing to do with each other. The connection comes through the so-called Hamiltonian representation theorem \citep{polterovich2012geometry}, which states that any symplectic diffeomorphism from $\mathcal{C} \subseteq \R^{2d} \to \R^{2d}$ can be written as the iteration of the following \emph{Hamiltonian} system of ODEs for some (time-dependent) Hamiltonian $H(x,v,t)$:
\begin{equation}
\label{eqn:ode_hamiltonion}
\begin{cases}  
\frac{dx}{dt} = \frac{d}{dv} H(x,v,t) \\ 
\frac{dv}{dt} = -\frac{d}{dx} H(x,v,t)
\end{cases}
\end{equation}
In fact, in our theorem, we will use techniques inspired by those in  \cite{turaev2002polynomial}, who shows: 
\begin{theorem}[\cite{turaev2002polynomial}]
For any function $H(x,v, t):\mathbb{R}^{2d}\times \R_{\ge 0} \to \mathbb{R}$ which is polynomial in $(x,v)$, there exists a polynomial $V(x,v,t)$, s.t. the time-$\tau$ map of the system 
\begin{equation}
\begin{cases}  
\frac{dx}{dt} = \frac{\partial}{\partial v} H(x,v,t) \\ 
\frac{dv}{dt} = -\frac{\partial}{\partial x} H(x,v,t)
\end{cases}
\label{eq:turaev}
\end{equation}
is uniformly $O(\tau^2)$-close to the time-$2\pi$ map of the system  
\begin{equation}
\label{eq:turaev_approx}
\begin{cases}  
\frac{dx}{dt} = v \\ 
\frac{dv_j}{dt} = -\Omega_j^2 x_j - \tau  \frac{\partial}{\partial x_j} V(x,t)
\end{cases}
\end{equation}
for some integers $\{\Omega_i\}_{i=1}^d$. 
\end{theorem}

We will prove a generalization of this theorem that applies to underdamped Langevin dynamics.


%The main idea is that each ``timestep'' of the diffusion can be simulated even if the  



==> proof_sketch.tex <==
\section{Proof Sketch of Theorem \ref{thm:main_universal_approx}}
\label{sec:proof_sketch}

\subsection{Overview of strategy}
\label{subsec:overview_strategy}

As a starting point, our approach to prove Theorem \ref{thm:main_universal_approx} involves flipping the problem statement around, and showing that there is a well-conditioned affine-coupling network $g'$ such that $g'_\# p \approx \mathcal{N}(0,\id_{2d})$, where $p$ is the target log-concave distribution. Since affine-coupling networks are invertible, we can then invert $g'$ to get the required network. Informally, if $g$ is the inverse of $g'$ with a bounded Lipschitz constant and $g'_\# p \approx \mathcal{N}(0,\id_{2d})$, it follows that $g_\# \mathcal{N}(0,\id_{2d}) \approx p$. We formalize this toward the end of this section.

% \hlnote{Need to work out how truncation interacts with taking the inverse.}

% This argument can be formalized as follows. Suppose that $W_1(g'_\#p, \mathcal{N}(0,\id_{2d})) \le \epsilon$. Then, by the definition of Wasserstein-1 distance, there is a coupling $(X,Y) \sim \gamma$ with marginals $g'_\#p$ and $\mathcal{N}(0,\id_{2d})$ such that  
% \[ \int \norm{x-y}_2 \,d\gamma \le \epsilon. \]
% Now, consider the coupling of $p$ and $ g_\# \mathcal{N}(0,\id_{2d})$ obtained by applying $g$ to $(X,Y) \sim \gamma$, i.e. $(g_\#X, g_\#Y)$ where $g$ is the inverse of $g'$. \hlnote{Will need to argue that $g$ stays inside the region where the map is well-conditioned. (depends on how you define truncation)} Then we have
% \begin{equation}
% \label{e:inversion_bound}
% W_1(p, g_\# \mathcal{N}(0,\id_{2d})) \le \int \norm{g(x)-g(y)}_2 \,d\gamma \le \Lip(g) \int \norm{x-y}_2\, d\gamma \le \Lip(g) \epsilon
% \end{equation}
% \Cnote{say something about Lip(g)}

Therefore, from now on, we will assume that the initial distribution $p_0 = p$, and the target distribution $p^* = \mathcal{N}(0,\id_{2d})$. % (also justifying the Langevin equations defined above.)
Our proof strategy comprises of two important steps:
\begin{enumerate}
    \item First, we show that not only does running underdamped Langevin (equations \eqref{e:m-uld}) converge to a sample from the target distribution $p^*$, but also the resulting flow-map is well-conditioned (Lemma \ref{lemma:underdamped_conditioning} below). Here, by flow-map, we mean the map which assigns each $x$ to its evolution over a certain amount of time $T$ according to the equations specified by \eqref{e:m-uld}. % \anote{say what the "flow map" is in English. it's not so clear what you mean}
    \item Next, we break the simulation of underdamped Langevin dynamics for a certain time $T$ into chunks of size $\tau$, and show that the flow-map over each $\tau$-sized chunk of time can be approximated well by a composition of affine-coupling maps (Lemma \ref{l:ode_approx} below). To show this, we consider a more general Hamiltonian system than the one in \cite{turaev2002polynomial}, which accommodates for \emph{underdamped} Langevin dynamics. We then show that the flow-map of this generalized Hamiltonian system can be cast as a composition of affine-coupling blocks using similar arguments as theirs.
\end{enumerate}

\subsection{Underdamped Langevin is well-conditioned}
\label{subsec:underdamped_conditioning}
%To begin, we state the following lemma, which concretizes the first step of our argument:
Consider running underdamped Langevin dynamics with stationary distribution equal to the standard gaussian, started at a log-concave distribution with bounded condition number $\ka$. 
The following lemma says that the flow map is well-conditioned, with condition number depending polynomially on $\ka$.
\begin{lemma}
\label{lemma:underdamped_conditioning}
Consider underdamped Langevin dynamics~\eqref{e:m-uld}
%\eqref{e:m-uld-1}--\eqref{e:m-uld-2} 
%smooth f, dissipative
with $\ze=1$, friction coefficient $\ga<2$ and starting distribution $p$ which satisfies all the assumptions in Theorem~\ref{thm:main_universal_approx}. Let $T_t$ denote the transport \fixme{flow?} map from time $0$ to time $t$ induced by~\eqref{e:m-uld-3-0}. Then for any $x_0,v_0 \in \R^d$ and unit vector $w$, the directional derivative of $T_t$ at $x_0,v_0$ in direction $w$ satisfies
\begin{align*}
    %\rc{e^{1/2}\min\{1,\sqrt{\ka-1}\}}
    \pa{1+\fc{2+\ga}{2-\ga}(\ka-1)}^{-2/\ga} \le 
    \ve{D_w T_t(x_0)} \le \pa{1+\fc{2+\ga}{2-\ga}(\ka-1)}^{2/\ga}.
    %\sqrt\ka.
    %e^{1/2}\min\{1,\sqrt{\ka-1}\}.
\end{align*}
Therefore, the condition number of $T_t$ is bounded by $\pa{1+\fc{2+\ga}{2-\ga}(\ka-1)}^{4/\ga}$.
\end{lemma}
We sketch the proof below; a complete proof is in Section~\ref{s:conditioning}.

First, using~\eqref{e:m-uld-3-0} and the chain rule shows that the Jacobian of the flow map at $x_0$, $D_t=DT_t(x_0)$, satisfies 
\begin{align}
    \label{e:jh-0}
    \ddd tD_t &=\matt{O}{I_d}{-I_d}{-\ga I_d} \nb^2 (\ln p_t - \ln p) D_t,
\end{align}
i.e., it is bounded by the difference of the Hessians of the log-pdfs of the current distribution and the stationary distribution. We will show that $\nb^2\ln p_t$ decays exponentially towards $\nb^2\ln p = \id_{2d}$.

To accomplish this, consider how $\nb^2 \ln p_t$ evolves if we replace~\eqref{e:m-uld} by its discretization, 
\begin{align*}
    \td x_{t+\eta} &= \td x_t + \eta \td v_t\\
    \td v_{t+\eta} &= (1-\eta \ga) \td v_{t} - \eta \td x_t + \xi_t,\quad \xi_t\sim N(0,2\eta \id_d).
\end{align*}
Note that because the stationary distribution is a gaussian, $\nb U(x_t) = x_t$ and the above equations take a particularly simple form: we apply a linear transformation to $\coltwo{ \td x_t}{\td v_t}$, and then add gaussian noise, which corresponds to convolving the current distribution by a gaussian.
We keep track of upper and lower bounds for $\nb^2 \ln p_t$, and compute how they evolve under this linear transformation and convolution by a gaussian. 
Taking $\eta\to 0$, we obtain differential equations for the upper and lower bounds for $\nb^2 \ln p_t$, which we can solve. A Gronwall argument shows that these bounds decay exponentially towards $\nb^2\ln p = \id_{2d}$. The decay rate is inverse polynomial in $\ka$.

From~\eqref{e:jh-0}, we then obtain that the condition number of $D_t$ is bounded by the integral of a exponentially decaying function, and hence is bounded independent of $t$. In particular, we may take $t$ large enough so that $p_t$ is $\ep$-close to the stationary distribution. Because the decay rate of the exponential is $\rc{\poly(\ka)}$, the bound is $\poly(\ka)$. 

Note that we vitally used the fact that the stationary distribution $p$ is a standard gaussian, as our argument requires that $\nb^2 \ln p$ be constant everywhere.

\subsection{ODE approximation by affine-coupling blocks}

As mentioned above, our proof strategy involves analyzing a more generalized version of the Hamiltonian system considered in \cite{turaev2002polynomial}, which has been specified in \eqref{eqn:turaev_hamiltonian} above. In particular, the system that we are concerned with is the following:
\begin{equation} 
\begin{cases}  
\frac{dx}{dt} = \frac{\partial}{\partial v} H(x,v,t) \\ 
\frac{dv}{dt} = -\frac{\partial}{\partial x} H(x,v,t) - \gamma \frac{\partial}{\partial v} H(x,v,t)
\end{cases}
\label{eq:underdamped_hamiltonian}
\end{equation}
Note that substituting $H(x,v,t) = \ln p_t(x,v) - \ln p^*(x,v)$ above gives us the underdamped Langevin dynamics. The following lemma first establishes that it suffices to focus on the Hamiltonian $H$ being polynomial in $x,v$:

\begin{definition}
Let $\mathcal{C} \subseteq \R^n$ be a compact set. Let $f,g : \mathcal{C} \to \R$ be two continuously differentiable functions. Then we say that $f,g$ are uniformly $\epsilon$-close over $\mathcal{C}$ in $C^1$ topology if
\[ \sup_{x \in \mathcal{C}} \brac{\norm{f(x) - g(x)} + \norm{Df(x) - Dg(x)}} \le \epsilon \]
\end{definition}

\begin{lemma}
\label{lemma:poly_approx_smooth_fn}
    Let $\mathcal{C} \subset \R^n$ be a compact set. For any $C^2$ function $H:\R^n \to \R$, and any $\epsilon > 0$, there is a multivariate polynomial $P:\R^n \to \R$ such that $P,H$ are uniformly $\epsilon$-close over $\mathcal{C}$ in $C^1$ topology.
    \todo{citation for this}
\end{lemma}
    
Proceeding ahead, let $T_{t,\tau}$ denote the time-$\tau$ flow-map of \eqref{eq:underdamped_hamiltonian} from time $t$ to time $t+\tau$. Lemma \ref{lemma:poly_ode_approx} below shows that instead of flowing the ODE given by \eqref{eq:underdamped_hamiltonian} over this chunk, we can instead run a different ODE, such that the time-$\tau$ flow-maps corresponding to both these ODEs are $O(\tau^2)$-close. 
    
\begin{lemma}
\label{lemma:poly_ode_approx}
Let $\mathcal{C} \subset \R^n$ be a compact set. For any function $H(x,v, t):\mathbb{R}^{2d} \to \mathbb{R}$ which is polynomial in $(x,v)$, there exist polynomial functions $J, F, G$, s.t. the time-$(t_0,t_0+\tau)$ flow map of the system
\begin{equation} 
\begin{cases}  
\frac{dx}{dt} = \frac{\partial}{\partial v} H(x,v,t) \\ 
\frac{dv}{dt} = -\frac{\partial}{\partial x} H(x,v,t) - \gamma \frac{\partial}{\partial v} H(x,v,t)
\end{cases}
\label{eq:hamiltonian}
\end{equation}
is uniformly $O(\tau^2)$-close in $C^1$ over $\mathcal{C}$ topology to the time-$2\pi$ map of the system
\begin{equation}
\label{eqn:affine_coupling_ode}
\begin{cases}  
\frac{dx}{dt} = v - \tau F(v,t) \odot x \\ 
\frac{dv_j}{dt} = -\Omega_j^2 x_j - \tau J_j(x,t) - \tau v_j G_j(x,t)
\end{cases}
\end{equation}
Here, $\odot$ denotes component-wise product, and the constants inside the $O(\cdot)$ depend on $\mathcal{C}.$
\end{lemma}
\Cnote{say few lines about the proof, reduce by moving to sin/cos basis to system of lin eqs; prove system is full-rank by exploiting structure of terms, also say that discretization of new ODE is affine-coupling}
    
Finally, consider discretizing the newly constructed ODE \eqref{eqn:affine_coupling_ode} into small steps of size $\eta$ i.e.
\begin{equation}
\label{eqn:discretized_affine_coupling_ode}
\begin{cases}  
x_{n+1}= x_n +  \eta(v_n - \tau F(v_n,\eta n) \odot x_n) \\ 
v_{n+1, j} = v_{n,j} -\eta(\Omega_j^2 x_{n,j} - \tau J_j(x_n,\eta n) - \tau v_{n,j} G_j(x_n,\eta n))
\end{cases}
\end{equation}
Note that each step above can be written as a composition of affine coupling blocks \todo{flesh it out in appendix?} given by
\[ (x_n, v_n) \mapsto (x_n, v_{n+1}) \mapsto (x_{n+1},v_{n+1}) \]
Note that we can write recover $v_n$ from $(x_n, v_{n+1})$. Further, observe that all the maps $F,G,J$ as defined in \eqref{e:fgj_defintions} are polynomials in $x$ or $v$, and hence, these affine-coupling blocks have polynomial \fixme{activations}. Then, the following lemma bounds the error resulting from the discretization:
\begin{lemma}[Euler's discretization method]
    \label{lemma:discretization_error}
    Let $\mathcal{C} \subset \R^n$ be a compact set. Consider discretizing the time from $0$ to $t$ into $\frac{t}{\eta}$ steps and performing the update given by \eqref{eqn:discretized_affine_coupling_ode} at each of these steps. Let the map obtained as a result of discretizing thus be denoted by $T'_t$ and let the original flow map be denoted by $T_t$. Then $T_t$ and $T'_t$ are uniformly $O(\eta)$ close over $\mathcal{C}$ in $C^1$ topology, and the constants inside the $O(\cdot)$ depend on $\mathcal{C}$.
\end{lemma}
    
\subsection{Simulating by breaking into $\tau$-sized chunks}
We are now ready to state the following lemma which says that the underdamped Langevin flow-map $T_\timethree$ can be written as a composition of affine-couplings maps:
\begin{lemma}
\label{l:ode_approx}
Let $\mathcal{C} \subset \R^{2d}$ be a compact set. Suppose that $T_\timethree(x,v)$ is the time-$\timethree$ flow-map of the ODE's below,
\begin{equation}
\label{eqn:ode_approx}
\begin{cases}  
\frac{dx}{dt} = \frac{\partial}{\partial v} H(x,v,t) \\ 
\frac{dv}{dt} = -\frac{\partial}{\partial x} H(x,v,t) - \gamma \frac{\partial}{\partial v} H(x,v,t)
\end{cases}
\end{equation}
where $H$ is $C^\infty$. Then for any $\epsilon,  \timethree \in \R_+$, there exists an integer $N = N(\epsilon, \timethree, \mathcal{C})$ 
\todo{explicit value of $N$ - upper bound? should be something like $2 * \frac{2\pi}{\eta} * \frac{\phi}{\tau}$}
and affine-coupling blocks $f_1, \ldots, f_N$ such that the composition $f = f_N \circ \cdots \circ f_1$ is $\epsilon$-close to $T_\timethree$ in the $C^1$ topology over $\mathcal{C}$, that is
\[ \sup_{x,v \in C} \left(\norm{T_\timethree(x,v) - f(x,v)} + \norm{DT_\timethree(x,v) - Df(x,v)} \right) \le \epsilon \]
\end{lemma}
\todo{do not get confused between this $\epsilon$ here and the $\epsilon$ in Theorem}

\todo{give an actual bound here -- does this required smallest eigenvalue of $T_t$ to be very large compared to epsilon?}
\begin{proof}
    From Lemma \ref{lemma:poly_approx_smooth_fn}, it suffices to focus on $H$ being a polynomial. We break the time $\timethree$ for which we want to flow the ODE given by \eqref{eqn:ode_approx} into $(n+1)$ small chunks of length $\tau$ i.e. let $\tau = \timethree / (n+1)$. Further, let $A_i = T_{i\tau,\tau}$. Then, the time-$\timethree$ flow map can be write as the composition of $n+1$ maps, that is
    \[ T_\timethree = T_{\timethree - \tau,\tau} \circ \cdots \circ T_{0,\tau} = A_n \circ \cdots \circ A_0 \]
    Let $S_i$ denote the time-$2\pi$ flow map obtained by running the ODE system \eqref{eqn:affine_coupling_ode} from Lemma \ref{lemma:poly_ode_approx} above which approximates the map $T_{i \tau, (i+1)\tau} = A_i$. Further, let $S'_i$ denote the map obtained by discretizing the ODE system as in \eqref{eqn:discretized_affine_coupling_ode} with step size $\eta$. Then, we have that for each $i$,
    \begin{align*}
    \norm{S'_i - A_i}_\infty  &\le \|S'_i - S_i + S_i - A_i\|_\infty \\
    &\le \|S'_i - S_i\|_\infty + \|S_i - A_i\|_\infty \\
    &\le O(\eta) + O(\tau^2) \quad \text{(by Lemmas \ref{lemma:discretization_error} and \ref{lemma:poly_ode_approx})}
    \end{align*}
    Therefore,
    \begin{align*}
        \norm{A_n \circ \cdots \circ A_0 - S'_n \circ \cdots \circ S'_0}_\infty
        & \le \norm{A_n \circ \cdots \circ A_1 \circ A_0 - A_n \circ \cdots \circ A_1 \circ S'_0}_\infty \\
        & + \norm{A_n \circ \cdots \circ A_1 \circ S'_0 - S'_n \circ \cdots \circ S'_1 \circ S'_0}_\infty \tag{by triangle inequality}\\
        & \le \norm{D T_{\tau, \timethree - \tau}} \norm{S'_0 - A_0}_\infty + \norm{A_n \circ \cdots \circ A_1 - S'_n \circ \cdots \circ S'_1}_\infty\\
        & \le \sum_{i=1}^{n+1} \norm{D T_{i\tau, \timethree -i \tau}} \norm{S'_{i-1} - A_{i-1}}_\infty
        \tag{by induction}
        \\
        & \le (n+1)\cdot (O(\eta) + O(\tau^2)) = \fc{\timethree}{\tau} \cdot {(O(\eta) + O(\tau^2))} = O\left(\frac{\eta}{\tau}\right) + O(\tau)
    \end{align*}
    where in the last step, we have assumed that $\norm{D T_{i \tau, \timethree - i \tau}}$ is bounded for all $i$, which follows from Lemma \ref{} above. Now, choosing $\eta = O(\tau^2)$ makes the error $O(\tau)$. Finally, we can choose $\tau$ small enough so that the error is smaller than $\epsilon$.
    
     Concretely, we can write each $S'_i$ as a composition of affine-coupling maps (which constitute the $f_1, \dots, f_N$ in the lemma statement. In this manner, we can compose these compositions of affine coupling maps over each $\tau$-sized chunk of time so as to get a map which is overall close to the required flow map.
\end{proof}

\subsection{Putting it together/inverting}
The previous sections established that \fixme{for any $t$ and any compact set $\mathcal{C}$, there is a polynomial-affine-coupling network $f$ such that} $T_t$ and $f$ are uniformly close over $\mathcal{C}$. \fixme{We will now pick appropriate values of $t$ and $\mathcal{C}$ such that $W_1(f_\# (p_0 |_{\mathcal{C}}), p^*) \le \epsilon$ where $p^* = \mathcal{N}(0,\id)$}.
%and it remains to show that the pushforwards of $p_0$ through these maps, namely, $f_\#(p_0)$ and ${T_t}_\#(p_0)$ are also close in Wasserstein distance. To do this, we will require the following lemma, which states that for compact sets $\mathcal{C}$ having a bulk of mass of a distribution $p$, $p$ and $p|_\mathcal{C}$ are close:
First, using \cref{thm:L-ma_mcmc}, for $\phi > -10 \log \epsilon + \log 2 + \log \mathcal{L}[p_0]$, $\KL(T_{\phi\#} (p_0), p^*) \le \frac{\epsilon^2}{2}$. Then using
%\fixme{
\hlnote{Replaced with easier to use theorem.}
\begin{theorem}[\citet{talagrand1996transportation,otto2000generalization}]
    If $p$ is a distribution on $\R^d$ satisfying a log-Sobolev inequality with constant $c$, then $p$ satisfies a \emph{transportation cost inequality}: For every distribution $q$ on $\R^d$ with finite second moment, 
    $W_1(p,q)^2 \le W_2(p,q)^2\le 2c KL(q \Vert p)$. In particular, when $p$ is standard Gaussian, the inequality holds for $c=1$.
\end{theorem}
%alternatively, Talagrand inequality for p gaussian
%}
we get that $W_1(T_{\phi\#} (p_0),p^*) \le \epsilon$. Now, we establish a bound on wasserstein distance between a log-concave distribution and its truncation on a compact set

\begin{lemma}
    \label{l:conditional_wasserstein}
    Let $p$ be a strongly log-concave distribution satisfying $- \nabla^2 \ln p \succeq \id$ with mode $x_0$ (that is, $\argmin_{x \in \R^d} -\ln p (x) = x_0$). Let $g$ be a function with global Lipschitz constant $L$. Then for any $\epsilon > 0$, there exists $\delta, R > 0 \in \R$ such that for any compact set $\mathcal{C}$ for which $\mathbb{P}_{x \sim p} [x \in \mathcal{C}] > 1 - \delta$ and $\mathcal{C} \subseteq B(x_0,R)$, the Wasserstein distance between $g_\# p$ and $g_\#(p|_{\mathcal{C}})$ is at most $\epsilon$.
\end{lemma}


Now, we fix a compact set $\mathcal{C}$ satisfying \cref{l:conditional_wasserstein} with $g = T_\phi$, and $g(x) = x$ for $\epsilon$. \Snote{why does such a $\mathcal{C}$ exist?}. Therefore, on this compact set $W_1({T_\phi}_\# (p_0 |_{\mathcal{C}}), {T_\phi}_\#(p_0)) \le \epsilon$.  Using Lemma \ref{l:ode_approx}, we can find an affine coupling network $f$ that is uniformly $\epsilon$ close to $T_\phi$ on the compact set $\mathcal{C}$. Now, we show that $W_1(f_\# (p_0 |_{\mathcal{C}}), {T_\phi}_\# (p_0 |_{\mathcal{C}})) \le \epsilon$.


% For simplicity of notation, let $\mu= f_\#(\mathcal{N}(0, \id))$ and $\nu={T_t}_\#(\mathcal{N}(0, \id)))$. Let $\Gamma(\mu, \nu)$ denote the collection of all measures on $C \times C$ with marginals $\mu$ and $\nu$ on the first and second factors respectively. \todo{confirm that the space of measures is $C \times C$} By definition of the Wasserstein-1 distance,
% \begin{align}
%     W_1(\mu, \nu) = \inf_{\gamma \in \Gamma(\mu, \nu)} \; \int_{C \times C}\|x-y\|_2\, d\gamma(x,y)
% \end{align}
Consider the coupling $\gamma'$, where a sample $(x,y) \sim \gamma'$ is generated as follows: first, we sample $z \sim p_0|_\mathcal{C}$, and then compute $x=f(z)$, $y=T_t(z)$. By definition of the pushforward, the marginals of $x$ and $y$ are $f_\#(p_0|_\mathcal{C})$ and ${T_t}_\#(p_0|_\mathcal{C})$ respectively. However, we know that for this $\gamma'$, from Lemma \ref{l:ode_approx}, $\|x-y\|_2 \le \epsilon$ uniformly. Thus, we can conclude that
\begin{align}
    W_1(f_\#(p_0|_\mathcal{C}), {T_t}_\#(p_0|_\mathcal{C})) &\le \int_{\R^d \times \R^d}\|x-y\|_2 \,d\gamma'(x,y) \\
    &\le \int_{\R^d \times \R^d}\epsilon\, d\gamma'(x,y)
    %=  \epsilon \int_{C \times C}\ d\gamma'(x,y)\\
    %&
    =\epsilon
\end{align}

Putting all these together, we get by triangle inequality
\[ W_1(f_\# (p_0 |_{\mathcal{C}}), p^*) \le 3 \epsilon \]

Let $\mathcal{C}' = f(\mathcal{C})$. Assuming that $\mathcal{C}'$ satisfies conditions of \cref{l:conditional_wasserstein} for $p^* = \mathcal{N}(0,\id)$, $g(x) = x$ and $\epsilon$ for some choice of
$\delta, R$, we have
\[ W_1(p^*, p^* |_{\mathcal{C}'}) \le \epsilon \]
which gives by triangle inequality 
\[ W_1(f_\# (p_0 |_\mathcal{C}), p^* |_{\mathcal{C}'}) \le 4 \epsilon \]


\paragraph{Handling the inverse.}
Now, taking pushforwards of both the distributions through $g = f^{-1}$. The wasserstein distance can be bounded in a similar manner as above. Since $W_1(f_\# (p_0 |_\mathcal{C}), p^* |_{\mathcal{C}'}) \le 4 \epsilon$, let $\gamma = (x,y)$ be a coupling such that
\[ \int \norm{x-y}_2 \,d\gamma \le 4 \epsilon. \]
Now consider the coupling $\gamma'$ of $p_0 |_\mathcal{C}$ and $g_\# (p^* |_{\mathcal{C}'})$ given by applying $g$ to $(x,y)$. Then we have

\begin{equation}
\label{e:inversion_bound}
W_1(p_0 |_\mathcal{C}, g_\# (p^* |_{\mathcal{C}'})) \le \int \norm{g(x)-g(y)}_2 \,d\gamma \le \Lip_\mathcal{C'}(g) \int \norm{x-y}_2\, d\gamma \le 4 \Lip_{\mathcal{C'}}(g) \epsilon
\end{equation}

\[ W_1(p_0 |_\mathcal{C}, g_\# (p^* |_{\mathcal{C}'})) \le 4 \Lip(g) \epsilon \]
as $f$ is well-conditioned, we have a bound on $\Lip(g)$ over the compact set $\mathcal{C}'$, we get the result (by appropriate choice of $\epsilon$).

% \citet{ma2019mcmc} show that $\KL(p_T \Vert p^*) \le \frac{\epsilon^2}{2}$ for $T \ge -\log \epsilon + 0.5 \log 2$. Note that $p^*$ here is a standard Gaussian. This gives us a bound on the Wasserstein distance using the following.

% % \begin{theorem}[\citet{BOBKOV19991}]
% %     \label{thm:bobkov-gotze}
% %     Let $p,q: \R^d \to \R^+$ be two distributions s.t. for every $1$-Lipschitz $f:\R^d \to \R^+$ and $X \sim p$, $f(X)$ is $c^2$-subgaussian. Then, we have $W_1(p,q)^2 \le 2 c^2 KL(q \Vert p)$.
% %     \hlnote{There's a version of this theorem for any $p$ satisfying a log-Sobolev inequality. Then you don't have to go through the extra step of verifying the condition.}
% % \end{theorem}



% We apply this theorem with $p = p^*$ and $q = p_T$, giving 
% %Because push-forwards of the standard Gaussian through an $L$-lipschitz function are $L^2$-subgaussian (Theorem 5.2.2 of \citet{vershynin2018high}),  \cref{thm:bobkov-gotze} above goes through with $c=1$, giving us that
% \[ W_1(p_T,p^*)^2 \le 2\KL(p_T \Vert p^*) \le \epsilon^2 \]
% which implies $W_1(p_T,p^*) \le \epsilon$ for $T \ge \frac{-\log \epsilon + \log 2}{4}$. \hlnote{Different from above.}

% By the triangle inequality, we get that $W_1(f_\#p_0, p^*) \le 2 \epsilon$.

% #Lemma 19 proof
% \begin{proof}
% Note that since $-\ln p$ is $1$-strongly convex and $x_0$ is the mode of $p$, we get
% \[ -\ln p(x) \ge -\ln p(x_0) + \frac{\norm{x - x_0}^2}{2} \]
% This gives us the tail bound
% \[ p(x) \le p(x_0) e^{-\frac{\norm{x - x_0}^2}{2}}. \]

% Let $q$ denote the distribution obtained by conditioning $p$ on $\mathcal{C}$, that is, $q(x) \propto p(x)$ if $x \in \mathcal{C}$ and $q(x) = 0$ otherwise. Consider the following coupling $\gamma = (x,y)$ as follows: draw $x$ from $p$. If $x \in \mathcal{C}$ then $y = x$ otherwise, draw $y$ according to $q$. Since $p$ and $q$ are proportional inside $\mathcal{C}$, this distribution has the correct marginals. Now, we bound the Wasserstein distance as follows:
% \begin{align}\nonumber
%     W_1(p,q)
%     & \le \int_{\R^d \times \mathcal{C}} \norm{x-y}\, d \gamma
%      \le \int_{\R^d \setminus \mathcal{C} \times \mathcal{C}} (\norm{x - x_0} + \norm{x_0 - y})\, d\gamma \\
%     & \le \int_{\R^d \setminus \mathcal{C}} (\norm{x-x_0} + R)\, dp
%      \le \int_{\R^d \setminus \mathcal{C}} \norm{x - x_0} \, dp + R\delta
%      \label{e:tail}
% \end{align}
% %Since $\int_{\R^d} \norm{x - x_0} \, dp < \infty$, we have that
% Now we claim that
% \begin{align*}
% \lim_{\delta \to 0^+}\sup_{\mathcal{C}: p(\mathcal{C}) > 1-\delta} \int_{\R^d \setminus \mathcal{C}} \norm{x - x_0} \, dp = 0.
% \end{align*}
% To see this, note that the sup is attained when we take $\mathcal C$ such that $\R^d\setminus \mathcal C$ is concentrated on the largest possible values of $\ve{x-x_0}$, i.e., when $\mathcal C = B(x_0,R(\de))$, for $R(\de)$ chosen so this has mass $1-\de$. By the dominated convergence theorem, $\lim_{\de\to 0^+}\int_{\R^d \setminus B(x_0,R(\de))} \ve{x-x_0}\,dp = 0$.

% Thus, both the terms in RHS in~\eqref{e:tail} are decreasing as functions of $\delta$. Consequently, we can find $\delta$ small enough such that each term is smaller than $\frac{\epsilon}{2}$, so that the overall RHS becomes smaller than $\epsilon$, giving us the required result.

% \paragraph{Handling the inverse.}
% The argument about inversion can be formalized as follows. Suppose that $W_1(g'_\#p, \mathcal{N}(0,\id_{2d})) \le \epsilon$. Then, by the definition of Wasserstein-1 distance, there is a coupling $(X,Y) \sim \gamma$ with marginals $g'_\#p$ and $\mathcal{N}(0,\id_{2d})$ such that  
% \[ \int \norm{x-y}_2 \,d\gamma \le \epsilon. \]
% Now, consider the coupling of $p$ and $ g_\# \mathcal{N}(0,\id_{2d})$ obtained by applying $g$ to $(X,Y) \sim \gamma$, i.e. $(g_\#X, g_\#Y)$ where $g$ is the inverse of $g'$. \hlnote{Will need to argue that $g$ stays inside the region where the map is well-conditioned. (depends on how you define truncation)} Then we have
% \begin{equation}
% \label{e:inversion_bound}
% W_1(p, g_\# \mathcal{N}(0,\id_{2d})) \le \int \norm{g(x)-g(y)}_2 \,d\gamma \le \Lip(g) \int \norm{x-y}_2\, d\gamma \le \Lip(g) \epsilon
% \end{equation}
% \Cnote{say something about Lip(g)}

% \fixme{First, observe that if $U = -\ln p$, then $U$ is strongly convex, and if $x_0$ is the minima for $U$, then by strong-convexity, we get that 
% \[ U(x) \ge U(x_0) + \frac{\norm{x-x_0}^2}{2} \ge \frac{\norm{x}^2}{4} - 4\norm{x_0}^2 + U(x_0) \]
% \begin{align*}
%     \norm{x-x_0}^2 & \ge \norm{x}^2 - 2 \norm{x}\norm{x_0} + \norm{x_0}^2 \\
%     & \ge \norm{x}^2 - 2 \max(\norm{x}, 4 \norm{x_0}) \max(\norm{x_0}, 1/4 \norm{x}) + \norm{x_0}^2 \\
%     & = \norm{x}^2 - 8 \max(\norm{x}/4, \norm{x_0})^2 + \norm{x_0}^2\\
%     & \ge \norm{x}^2 - 8 \brac{\norm{x}^2/16 + \norm{x_0}^2} + \norm{x_0}^2 \\
%     & = \norm{x}^2/2 - 7 \norm{x_0}^2 
% \end{align*}

% \Snote{This is very hacky need a better bound here}
% This implies that
% \[ p(x) \le e^{-\frac{\norm{x}^2}{4} + c} \]
% for $c = -U(x_0) + 4 \norm{x_0}^2$.

% Let $q$ denote the distribution obtained by conditioning $p$ on $\mathcal{C}$, that is by truncating $p$ to $\mathcal{C}$ and re-normalizing. Now, consider the following coupling: draw $X$ from $p$. If $X \in \mathcal{C}$, then $Y = X$. Otherwise draw pick a random $Y$ according to $q$. Note that since $p$ and $q$ are proportional inside $\mathcal{C}$, the coupling $\gamma = (X,Y)$ has correct marginals. Then,
% \begin{align}
%     W_1(p,q)
%     & \le \int_{\R^d \times \mathcal{C}} \norm{X-Y}\, d \gamma\\
%     & \le \int_{\R^d \setminus \mathcal{C}} (\norm{x} + R)\, dp \\
%     & \le \int_{\R^d \setminus \mathcal{C}} \norm{x} dp + R \int_{\R^d \setminus \mathcal{C}}\, dp\\
%     & \le \int_{\R^d \setminus \mathcal{C}} \norm{x} e^{-\norm{x}^2/2 + c}\, dx + R \epsilon\\
%     & \le e^c \epsilon + R \epsilon
% \end{align}
% \Snote{need to add condition that integral of norm outside $\mathcal{C}$ is also $\epsilon$, and also $R \epsilon$ should be small}. For nice enough $\mathcal{C}$, this is really tiny, which gives us the result.
% \Snote{Might need two balls, $B(0,R_1) \subseteq \mathcal{C} \subseteq B(0,R_2)$}.
% }
%\end{proof}

==> technical_machinery.tex <==
%!TEX root=main.tex

\subsection{Log-Sobolev inequalities}
\label{s:log_sobolev_inequalities}

Though we don't explicitly use it in any substantive manner in this paper, we include the definition of a log-Sobolev inequality for completeness. 
%* for now to not break lemma numbering
\begin{definition}
A distribution $p:\R^d \to \R^+$ satisfies a \emph{log-Sobolev} inequality with constant $C > 0$ if $\forall g:\mathbb{R}^d \to \mathbb{R}$, s.t. $g^2, g^2 |\log g^2| \in L^1(p)$, we have  
\begin{equation}
    \mathbb{E}_p[g^2 \log g^2] - \mathbb{E}_p[g^2] \log \mathbb{E}_p[g^2] \leq 2C \mathbb{E}_p\|\nabla g\|^2 .
\end{equation}
\end{definition}
In the subarea of Markov diffusions (and in particular, designing sampling algorithms using diffusions), the interest in this quantity comes as it governs the convergence rate of \emph{overdamped} Langevin diffusion in the KL divergence sense. Namely, if $p_t$ is the distribution of overdamped Langevin after time $t$, one can show
\[\mbox{KL}(p_t || p) \leq e^{-Ct} \mbox{KL}(p_0 || p). \] 


\subsection{Expressing the discretization step in \Cref{eqn:discretized_affine_coupling_ode} as an affine coupling network}
\label{s:affine_coupling_comp}
We recall the definition of an affine-coupling block from \Cref{s:notation}. An affine coupling block is a map $f: \mathbb{R}^d \to \mathbb{R}^d$, s.t.   $f(x_S, x_{[d] \setminus S}) = (x_S, x_{[d] \setminus S} \odot s(x_S) + t(x_S))$ for some set of coordinates $S$, where $\odot$ denotes entrywise multiplication and $s,t$ are trainable (generally non-linear) functions.

Now, consider the map $(x_n, v_n) \mapsto (x_n, v_{n+1})$ given by
\begin{align*}
\begin{cases}
    x_n = x_n \\
    v_{n+1} = v_n \odot (1-\tau)G(x_n, \eta n) - \eta(\Omega^2 \odot x_n - \tau J(x_n, \eta n))
\end{cases}
\end{align*}
Then, this map $(x_n, v_n) \mapsto (x_n, v_{n+1})$ is an affine coupling block corresponding to the definition above with $s(x_n) = (1-\tau) \odot G(x_n, \eta n)$ and $t(x_n) = - \eta(\Omega^2 \odot x_n - \tau J(x_n, \eta n))$.

Next, consider the map $(x_n, v_{n+1}) \mapsto (x_{n+1}, v_{n+1})$ given by
\begin{align*}
\begin{cases}
    v_{n+1} = v_{n+1} \\
    x_{n+1}= x_n +  \eta(v_{n+1} - \tau F(v_{n+1},\eta n) \odot x_n) \\ 
\end{cases}
\end{align*}
Then, this map $(x_n, v_{n+1}) \mapsto (x_{n+1}, v_{n+1})$ is an affine coupling block corresponding to the definition above with $s(v_{n+1}) = 1-\eta \tau F(v_{n+1}, \eta n)$ and $t(v_{n+1}) = \eta v_{n+1}$.

The composition of the two maps above yields an affine coupling network $(x_n, v_n) \mapsto (x_{n+1}, v_{n+1})$ precisely as given by \Cref{eqn:discretized_affine_coupling_ode}. Note that the non-linearities $s,t$ in each of the blocks above are polynomials.

\subsection{Proof of \Cref{lemma:discretization_error}}
\label{s:discretization_error_proof}
We consider a more general ODE than the specific one in \eqref{eqn:affine_coupling_ode}, of the form
\begin{equation}
\label{eqn:affine_euler}
    \begin{cases}
    \frac{d}{dt}(x(t)) = f(x(t), v(t) ,t) \\
    \frac{d}{dt}(v(t)) = g(x(t), v(t), t)
    \end{cases}
\end{equation}
where $f,g$ are %\fixme{(smooth functions)} polynomials 
$C^2$ functions in $x,v,t$. Given a compact set $\mathcal C$, suppose that the solutions are well-defined for any $(x(0),v(0))\in \mathcal C$ up to time $T$.  
Consider discretizing these ODEs into steps of size $\eta$, as follows:
\begin{equation}
\label{eqn:discretized_affine_euler}
\begin{cases}
    \widetilde T_i^x(X_i) = X_{i+1} = X_i + \eta f(X_i, %V_i + \eta g(X_i, V_i, t_i)
    V_{i+1}
    , t_i) \\
    \widetilde T_i^v(V_i) = V_{i+1} = V_i + \eta g(X_i, V_i, t_i)
\end{cases}
\end{equation}
where $t_i = i \eta$. We call this the alternating Euler update. The actual flow maps are given by %\hlnote{The mean-value theorem only works for univariate case. In general write the error term as an integral}
\begin{equation}\label{e:actual-flow-exp}
\begin{cases}
    T_i^x(x_i) = x_{i+1} = x_i + \eta f(x_i, v_i, t_i) +
    \int_{i\eta}^{(i+1)\eta} \int_{i\eta}^t x''(s)\,ds\,dt\\
    %\frac{\eta^2}{2} \left. \frac{d}{dt} \right\vert_{t^*}\brac{f(x(t), v(t), t)} \\
    T_i^v(v_i) = v_{i+1} = v_i + \eta g(x_i, v_i, t_i) +
    \int_{i\eta}^{(i+1)\eta} \int_{i\eta}^t v''(s)\,ds\,dt%\frac{\eta^2}{2}\left. \frac{d}{dt} \right\vert_{t^*}\brac{g(x(t), v(t), t)}
\end{cases}
\end{equation}
We bound the local truncation error. 
This consists of two parts. First, we have the integral terms in~\eqref{e:actual-flow-exp}:
\begin{align}\label{e:lte1}
    \ve{\coltwo{\int_{i\eta}^{(i+1)\eta} \int_{i\eta}^t x''(s)\,ds\,dt}{\int_{i\eta}^{(i+1)\eta} \int_{i\eta}^t v''(s)\,ds\,dt}}
    &\le 
    \rc 2\eta^2   \max_{s\in [0,t_i]} \ve{\coltwo{x''(s)}{v''(s)}}
    .
\end{align}
Second we bound the error from using $\widetilde v_{i+1}:=v_i + \eta g(x_i,v_i,t_i)$ instead of $v_i$ in the $x$ update,
\begin{align}\nonumber
    \ve{\eta[f(x_i, v_i + \eta g(x_i,v_i,t_i), t_i) - f(x_i,v_i,t_i)]}
    &\le 
    \ve{\eta\int_0^\eta 
    %\pd{f}{v}
    D_vf
    (x_i,v_i+sg(x_i,v_i,t_i),t_i) g(x_i,v_i,t_i)\,ds} \\
    &\le \eta^2 \max_{\mathcal C'} 
    \ve{D_vf} 
    %\ve{\pd{f}{v}}
    \max_{\mathcal C'} \ve{g} .
    \label{e:lte2}
\end{align}
% First, for $v$, \hlnote{should actually write $x_i,v_i$ together so we do max over both}
% \begin{align*}
%     \ve{\widetilde T_i^v(v_i) - T_i(v_i)}
%     &\le \rc 2 \eta^2 \max_{s\in [t_i,t_{i+1}]} \ve{v''(s)}.
% \end{align*}
% For $x$, we also bound the error from using $\widetilde v_{i+1}:=v_i + \eta g(x_i,v_i,t_i)$ instead of $v_i$,
% \begin{align*}
%     \ve{\widetilde T_i^x(x_i) - T_i(x_i)}
%     &\le 
%     \ve{\eta[f(x_i, v_i + \eta g(x_i,v_i,t_i), t_i) - f(x_i,v_i,t_i)]} + \rc 2 \eta^2 \max_{s\in [t_i,t_{i+1}]} \ve{x''(s)}\\
%     &\le 
%     \ve{\eta\int_0^\eta 
%     %\pd{f}{v}
%     D_vf
%     (x_i,v_i+sg(x_i,v_i,t_i),t_i) g(x_i,v_i,t_i)\,ds} +  \rc 2 \eta^2 \max_{s\in [t_i,t_{i+1}]} \ve{x''(s)}\\
%     &\le \eta^2 \max_{\mathcal C'} 
%     \ve{D_vf} 
%     %\ve{\pd{f}{v}}
%     \max_{\mathcal C'} \ve{g} + \rc 2 \eta^2 \max_{s\in [t_i,t_{i+1}]} \ve{x''(s)}
% \end{align*}
where %$\pd fv(x,v,t)\in \R^{d\times d}$
$D_v f(x,v,t)$ denotes the Jacobian in the $v$ variables (rather than the directional derivative), and where we define
\begin{align*}
\mathcal C' 
:&=
\{(x,v+sg(x,v,t),t): (x,v) = T_t(x_0,v_0) \text{ for some }(x_0,v_0)\in \mathcal C, 0\le s\le T\},
\end{align*}
which ensures that it contains $(x_i,v_i+sg(x_i,v_i,t_i),t_i)$ and $(x_i,v_i,t_i)$. The local truncation error is then at most the sum of~\eqref{e:lte1} and \eqref{e:lte2}.
%\hlnote{This may be larger than the original set, because the trajectory can leave $\mathcal C$! Need to argue it suffices to look at a set around the true trajectory.}

Supposing that $\coltwo fg$ is $L$-Lipschitz in $(x,v)\in \R^{2d}$ for each $t$, we obtain by a standard argument (similar to the proof for the usual Euler's method, see e.g.,~\cite[\S 16.2]{ascher2011first}) that the global error at any step is bounded by 
\begin{align}\label{e:alt-euler-bound}
    \ve{\coltwo{\widetilde x_i}{\widetilde v_i} - 
    \coltwo{x_i}{v_i}
    }
    &\le \eta \cdot \fc{e^{Lt_i}-1}L 
    \pa{
    \max_{\mathcal C'} \ve{D_v f}
    \max_{\mathcal C'} \ve{g} + \rc 2  \max_{s\in [0,t_i]} \ve{\coltwo{x''(s)}{v''(s)}}
    }.
\end{align}
In the case when $\coltwo fg$ is not globally Lipschitz, we show that we can restrict the argument to a compact set on which it is Lipschitz.
Let $\mathcal C''$ be a compact set which contains $\{(x,v,t):(x,v)=T_t(x_0,v_0)\text{ for some }(x_0,v_0)\in \mathcal C, 0\le s\le T\}$ in its interior. Apply the argument to $\hat{f}$ and $\hat g$ which are defined to be equal to $f, g$ on $\mathcal C''$, and are globally Lipschitz. Then the error bound applies to the system defined by $\hat f, \hat g$. Hence, for small enough step size, the trajectory of the discretization stays inside $\mathcal C''$, and is the same as that for the system defined by $f,g$. Then~\eqref{e:alt-euler-bound} holds for small enough $\eta$ and $L$ equal to the Lipschitz constant in $(x,v)$ on $\mathcal C''$.

%We will mention at the end how to adapt the argument when $\coltwo fg$ is not globally Lipschitz.

% Therefore, for any $x,v$, we have that
% \begin{align*}
%     \norm{T_i(x) - T'_i(x) + T_i(v) - T'_i(v)} &\le \norm{T_i(x) - T'_i(x)}  + \norm{T_i(v) - T'_i(v)}\\
%     &\hspace{-2cm}= \eta \norm{f(x, v + \eta g(x, v, t_i), t_i) -  f(x, v, t_i)} + \frac{\eta^2}{2}\left\|\left. \frac{d}{dt} \right\vert_{t^*}\brac{g(x, v, t)}\right\| \\
%     &\hspace{-2cm}= \eta \left\|f(x,v,t_i) + \eta g(x,v,t_i)\left.\frac{\partial}{\partial v}\right\vert_{v^*}f(x,v,t_i) - f(x,v,t_i)\right\|  \\
%     &\hspace{-2cm}\qquad\qquad+ \frac{\eta^2}{2}\left\|\left. \frac{d}{dt} \right\vert_{t^*}\brac{g(x, v, t)}\right\| \\
%     &\hspace{-2cm}= \eta^2 \left\| g(x,v,t_i)\left.\frac{\partial}{\partial v}\right\vert_{v^*}f(x,v,t_i)\right\| + \frac{\eta^2}{2}\left\|\left. \frac{d}{dt} \right\vert_{t^*}\brac{g(x, v, t)}\right\| \\
%     &\hspace{-2cm}\le \eta^2 \left\| g(x,v,t_i)\right\|\left\|\left.\frac{\partial}{\partial v}\right\vert_{v^*}f(x,v,t_i)\right\| + \frac{\eta^2}{2}\left\|\left. \frac{d}{dt} \right\vert_{t^*}\brac{g(x, v, t)}\right\| \\
%     &\hspace{-2cm}= O(\eta^2)
% \end{align*}
% where in the last step above, we assumed constant upper bounds on each norm term over the compact set $\mathcal{C}$, which hold because $f,g$ are smooth functions.

To get a bound in $C^1$ topology, we need to bound the derivatives of these maps as well. Let $T_{s,t}(x,v)$ %= (T^1_{s,t}(x,v), T^2_{s,t}(x,v))$ 
denote the flow map of system \eqref{eqn:affine_euler}. Let $h(x,v,t) = (f(x,v,t),g(x,v,t))$. Now, consider the system of ODEs
\begin{equation}
    \label{eqn:combined_odes}
    \begin{cases}
        \frac{d}{dt}(x(t))  = f(x(t),v(t),t)\\
        \frac{d}{dt}(v(t))  = g(x(t),v(t),t)\\
        \frac{d}{dt}(\alpha(t))  = D_{(x,v)}f (x(t),v(t),t) \coltwo{\alpha(t)}{\beta(t)}\\
        \frac{d}{dt}(\beta(t))  = D_{(x,v)}g (x(t),v(t),t)\coltwo{\alpha(t)}{\beta(t)}
    \end{cases}
\end{equation}
where $\alpha(t), \beta(t)$ are $d \times 2d$ matrices. Note that setting $\coltwo{\alpha(0)}{\beta(0)} = \id_{2d}$ and $\coltwo{\alpha(t)}{\beta(t)} = D_{(x,v)} T_{0,t} (x(0),v(0))$ satisfies \eqref{eqn:combined_odes} by \Cref{l:ode_derivative}.
%where $\alpha(t)$ is a $2d \times 2d$ matrix. Note that setting $\alpha(0) = \id$ and $\alpha(t) = D_{(x,v)} T_{0,t} (x(0),v(0))$ satisfies \eqref{eqn:combined_odes} by \Cref{l:ode_derivative}.

Now we claim that applying the alternating Euler update to $(x,\alpha), (v,\beta)$, the resulting $(\alpha_i,\beta_i)$ is exactly the Jacobian of the flow map that arises from alternating Euler applied to $x,v$. This means that we can bound the errors for $\alpha,\beta$ using the bound for the alternating Euler method.

The claim follows from noting that the alternating Euler update on $\alpha$, $\beta$ is
\begin{align*}
    \alpha_{i+1} &= 
    (\id_d,O) 
    + 
    D_{(x,v)}f(x_i,v_{i+1},t_i) \coltwo{\al_i}{\be_{i+1}}\\
    \beta_{i+1} &= 
    (O,\id_d) 
    + 
    D_{(x,v)}f(x_i,v_{i},t_i) \coltwo{\al_i}{\be_i},
\end{align*}
which is the same recurrence that is obtained from differentiating $X_{i+1},V_{i+1}$ in~\eqref{eqn:discretized_affine_euler} with respect to $X_0,V_0$, and using the chain rule.

Thus we can apply~\eqref{e:alt-euler-bound} to get a bound for the Jacobians of the flow map. The constants in the $O(\eta)$ bound depend on up to the second derivatives of the $x,v,\alpha,\beta$ for the true solution, Lipschitz constants for $\coltwo fg$, $D\coltwo fg$ (on a suitable compact set), and bounds for $D_vf, g, D_vD_{(x,v)}f, D_{(x,v)}g$  (on a suitable compact set).

\iffalse
    Now, consider the discretized updates in \eqref{eqn:discretized_affine_euler}. We will show that the derivative of the map $T_i'$ is $O(\eta^2)$ close to the discretized version of $\alpha(t)$ here. The discretized update for $\alpha(t)$ is given by
    \begin{equation}
        \label{eqn:euler_derivative}
        A_{i+1} = A_i + \eta D_{(x,v)}h(X_i,V_i,t_i) A_i =  \brac{\id_{2d} + \eta D_{(x,v)}h(X_i,V_i,t_i)} A_i
    \end{equation}
    
    On the other hand, $B_{i+1} = D(T_i' \circ \cdots \circ T_0') = DT_i'(X_i,V_i,t_i) B_i$. Now, we claim that 
    \[ \norm{\id_{2d} + \eta D_{(x,v)}h(X_i,V_i,t_i) - DT_i'(X_i,V_i,t_i)}_F = O(\eta^2) \]
    
    We will show this block by block. We will only show the explicit computations for the top-left $d \times d$ block, the rest will follow. Therefore, we have to show that
    \[ \norm{I_d + \eta D_x f(X_i,V_i,t_i) - D_x T'_i (X_i,V_i,t_i)}_F = O(\eta^2) \]
    
    Note that
    \begin{align*}
        D_x T'_i(x,v,t)
        &=  \id_d + \eta D_x f (x,v + \eta g(x,v,t) , t) + \eta D_v f(x, v + \eta g(x,v,t), t) \eta D_x g (x,v,t)\\
        & = \id_d + \eta D_x f(x,v,t) + \eta^2 g(x,v,t) D_v D_x f (x,v',t) + O(\eta^2)\\
        & = \id_d + \eta D_x f(x,v,t) + O(\eta^2)
    \end{align*}
    which follows since $g, D_v D_x f, D_x g$ are bounded on the compact set $\mathcal{C}$ as they are all smooth functions.
    
    This shows that the updates given in \eqref{eqn:discretized_affine_euler} and the derivatives of these maps are $O(\eta^2)$ close to the Euler updates of \eqref{eqn:combined_odes}. Since the Euler updates themselves have local error of $O(\eta^2)$ at each step, the exact same proof for the Euler method \citep{ascher2011first} will give us a global error bound of $O(\eta e^{O(t)})$, where $t$ is the total time. Since $t$ is bounded by $2 \pi$ here, we get a bound of $O(\eta)$ on the total error. 
    
    \Snote{here, the $\eta^2$ term is getting multiplied by the derivative. That should be fine, but might require a bound on the derivative of the flow map}
\fi

\subsection{Wasserstein bounds}
\label{s:wasserstein_bounds}

\begin{lemma}
\label{l:wasserstein_bound_1}
Given two distributions $p,q$ and a function $g$ with Lipschitz constant $L = \Lip(g)$,
\[ W_1(g_\# p, g_\# q) \le L W_1(p,q) \]
\end{lemma}
\begin{proof}
    Let $\epsilon >0$. Then there exists a coupling $(x,t) \sim \gamma$ such that 
    \[ \int \norm{x-y}_2 d\gamma(x,y) \le W_1(p,q) + \epsilon \]
    Consider the coupling $(x',y')$ given by $(x',y') = (g(x),g(y))$ where $(x,y) \sim \gamma$. Then
    \begin{align*}
        W_1(g_\# p, g_\#q)
        & \le \int \norm{g(x) - g(y)}_2 \, d\gamma(x,y) \\
        & \le \Lip(g) \int \norm{x - y} \, d\gamma(x,y)\\
        & \le L W_1(p,q) + L \epsilon.
    \end{align*}
    Since this holds for all $\epsilon > 0$, we get that
    \[ W_1(g_\# p, g_\#q) \le LW_1(p,q) \]
\end{proof}

\begin{lemma}
\label{l:wasserstein_bound_2}
Given two functions $f,g:\R^d \to \R^d$ that are uniformly $\epsilon_1$-close over a compact set $\mathcal{C}$ in $C^1$ topology, and a probability distribution $p$,
\[ W_1(f_\# (p|_\mathcal{C}), g_\# (p|_\mathcal{C})) \le \epsilon_1 \]
\end{lemma}
\begin{proof}
    Consider the coupling $\gamma$, where a sample $(x,y) \sim \gamma$ is generated as follows: first, we sample $z \sim p|_\mathcal{C}$, and then compute $x=f(z)$, $y=g(z)$. By definition of the pushforward, the marginals of $x$ and $y$ are $f_\#(p|_\mathcal{C})$ and $g_\#(p|_\mathcal{C})$ respectively. However, we are given that for this $\gamma$, $\|x-y\| \le \epsilon_1$ uniformly. Thus, we can conclude that
\begin{align*}
    W_1(f_\#(p|_\mathcal{C}), {g}_\#(p|_\mathcal{C})) &\le \int_{\R^d \times \R^d}\|x-y\|_2 \,d\gamma(x,y) \\
    &\le \int_{\R^d \times \R^d}\epsilon_1\, d\gamma(x,y)
    =\epsilon_1
\end{align*}
\end{proof}

\subsection{Proof of \Cref{l:conditional_wasserstein}}
\label{s:conditional_wasserstein_proof}
\begin{proof}
    Fix any $R > 0$, and set $\mathcal{C} = B(0, R)$. Consider the coupling $(X,Y) \sim \gamma$, where a sample $(X,Y)$ is generated as follows: we first sample $X \sim p^* = \mathcal{N}(0, \id_{2d})$. If $X \in B(0, R)$, then we set $Y=X$. Else, we draw $Y$ from $p^*|_\mathcal{C}$. Clearly, the marginal of $\gamma$ on $X$ is $p$. Furthermore, since $p^*$ and $p^*|_\mathcal{C}$ are proportional within $\mathcal{C}$, the marginal of $\gamma$ on $Y$ is $p^*|_\mathcal{C}$. Then, we have that
    \begin{align*}
        W_1(p^*, p^*|_\mathcal{C}) &\le \int_{\R^{2d} \times \mathcal C}  \|x-y\|d\gamma \\%\R^{2d}
        &%\hspace{-1.5cm}
        = \cancel{\int_{\mathcal{C} \times \mathcal{C}} \|x-y\|d\gamma} + %\cancel{\int_{\mathcal{C} \times \mathbb{R}^{2d}\setminus\mathcal{C}} \|x-y\|d\gamma} + 
        \int_{\mathbb{R}^{2d}\setminus\mathcal{C} \times \mathcal{C}}\|x-y\|d\gamma 
        %+ \cancel{\int_{\mathbb{R}^{2d}\setminus\mathcal{C} \times \mathbb{R}^{2d}\setminus\mathcal{C}}\|x-y\|d\gamma} 
        \\
        &%\hspace{-1.5cm}
        = \int_{\mathbb{R}^{2d}\setminus\mathcal{C} \times \mathcal{C}}\|x-y\|d\gamma \\
        &%\hspace{-1.5cm}
        \le \int_{\mathbb{R}^{2d}\setminus\mathcal{C} \times \mathcal{C}}(\|x\| + \|y\|)d\gamma \\
        &%\hspace{-1.5cm}
        \le \int_{\mathbb{R}^{2d}\setminus\mathcal{C} \times \mathcal{C}}(\|x\| + R)d\gamma \\
        &%\hspace{-1.5cm}
        \le \int_{\mathbb{R}^{2d}\setminus\mathcal{C} \times \mathcal{C}}(\|x\| + R)d\gamma \\
        &%\hspace{-1.5cm}
        = \int_{\R^{2d} \setminus \mathcal{C}} (\|x\| + R)dp^* \\
        &%\hspace{-1.5cm}
        \le \int_{\R^{2d} \setminus \mathcal{C}} 2\|x\|dp^* = \frac{2}{\sqrt{2\pi}}\int_{\R^{2d} \setminus \mathcal{C}} \|x\|e^{-\frac{\|x\|^2}{2}}dx
    \end{align*}
    Now, note that $\int_{\R^{2d} } \|x\|e^{-\frac{\|x\|^2}{2}}dx < \infty$.
    Hence, by the Dominated Convergence Theorem, \[\lim_{R\to \iy}\int_{\R^{2d} \setminus B(0,R)} \|x\|e^{-\frac{\|x\|^2}{2}}dx = 0.\]
    %Further, as $R$ increases, the set $\R^{2d} \setminus \mathcal{C}$ becomes smaller, and hence $\int_{\R^{2d} \setminus \mathcal{C}} \|x\|e^{-\frac{\|x\|^2}{2}}dx$ is a decreasing function in $R$. 
    Thus, given any $\delta >0$, we can choose $R$ large enough so that the integral above is smaller than $\delta$, which concludes the proof.
\end{proof}

\subsection{Derivatives of flow maps}
\label{s:derivative_flow_map}
We state and prove a technical lemma about the ODE that the derivative of a flow map satisfies.
\begin{lemma}
    \label{l:ode_derivative}
    Suppose $x_t = x(t)$ satisfies the ODE
    \[ \dot{x} = F(x,t) \]
    with flow map $T(x,t) : \R^n \times \R \to \R^n$. Suppose $\alpha(t)$ be the derivative of the map $x \mapsto T(x,t)$ at $x_0$, then $\alpha(t)$ satisfies
    \[ \dot{\alpha} = DF(x_t,t) \alpha \]
    with $\alpha(0) = \id$.
\end{lemma}
\begin{proof}
    Let $T_t(x) = T(x,t)$. Then $T_t$ satisfies
    \[ T_t(x_0) = \int_0^t F(x_s,s)\, ds. \]
	Differentiating, we get
	\begin{align*}
		\alpha(t) = DT_t(x_0)
		& = \int_0^t D(F(x_s,s)) \,ds \\
		& = \int_0^t DF(x_s,s) DT_s(x_0) \,ds \tag*{by chain rule}\\
		& = \int_0^t DF(x_s,s) \alpha(s)\, ds.
	\end{align*}
	Now, looking at the derivative with respect to $t$, we get
	\[ \dot{\alpha} = DF(x_t,t) \alpha, \]
	which is the required result.
\end{proof}

\subsection{Solving Perturbed ODEs}
\label{s:perturbation_analysis}
In this section, we state a result about finding approximate solutions of perturbed differential equations. Consider the ODE having the following general form:
\[ \dot{x} = Ax + \epsilon g(x,t) \]
The reason we are concerned with this ODE is that the ODE given by \Cref{eqn:affine_coupling_ode} has precisely this form, namely with $x \equiv \coltwo xv$, $A \equiv \begin{bmatrix} 0 & \id_d \\ -\text{diag}(\Omega^2) & 0 \end{bmatrix}$ and $\epsilon g(x,t)\equiv -\tau\begin{bmatrix} F(v,t) \odot x \\ J(x,t) + G(x,t) \odot v\end{bmatrix}$. 

Let $T^x: \R \times \R^n \to \R^n$ be the time $t$ flow map for this ODE. We will find a flow map $T^y: \R \times \R^n \to \R^n$ such that the maps $T_t^x$ defined by $T_t^x(x) = T^x(t,x)$ and the map $T_t^y$ defined by $T_t^y(y) = T^y(t,y)$ are uniformly $\epsilon$-close over $\mathcal{C}$ in $C^r$ topology for all $0 \le t \le 2 \pi$. That is, 
\[ \sup_{x} \qquad \norm{T_t^x(x) - T_t^y(x)} + \norm{DT_t^x(x) - DT_t^y(x)} + \dots + \norm{D^rT_t^x(x) - D^rT_t^y(x)}\]
is small, for all $t \in [0,2\pi]$. Here $D^r$ denotes the $r$-th derivative, and the norms are defined inductively as follows: for a $r$-tensor $\mathcal T$, we let $\ve{\mathcal T}=\sup_{\ve{u}=1}\ve{\mathcal Tu}$; here $\mathcal Tu$ is a $(r-1)$-tensor. (The choice of norm is not important; we choose this for convenience.)

% First, we will prove a couple of technical lemmas
\ifdefined\PROOF
\begin{lemma}
	\label{l:linear_ode_upper_bound}
	Any solution $w(t)$ of $\dot{w} \le aw + b$ for constants $a,b$ satisfies
	\[ w(t) \le \frac{b}{a} \brac{e^{at} - 1} + w(0)e^{at}. \]
\end{lemma}
\begin{proof}
	The solution of the corresponding differential equation is given by using an integrating factor.
	\begin{align*}
		\dot{w} - aw & \le b \\
		\implies \dot{w}e^{-at} - awe^{-at} & \le be^{-at} \\
		\implies \frac{d}{dt} (we^{-at}) & \le be^{-at} \\
		\implies w(t)e^{-at} - w(0) & \le \frac{b}{a} \brac{1 - e^{-at}} \\
		\implies w(t) & \le \frac{b}{a} \brac{e^{at} - 1} + w(0)e^{at} 
	\end{align*}
	This proves the bound that we want.
\end{proof}
\fi

The following lemma formalizes this:
\begin{lemma}
\hlnote{More general version of below}
   	Consider the ODE's
	\begin{align}
	\label{e:ode-perturb-orig}
	\ddd t x(t) &= F(x(t),t) + \epsilon G(x(t),t)\\
	\nonumber
	\ddd t y_0(t) &= F(y_0(t),t)\\
	\nonumber 
	\ddd t y(t) &= F(y(t),t) + \ep G(y_0(t),t) %\tag{\fixme{removed $\epsilon$}}
	\end{align}
	such $F,G:\R^n\times \R\to \R^n$ are in $C^{r+1}$. \hlnote{Modified so that $y=y_0+\ep y_1$ in the specialization} 
	Let $\mathcal C\subseteq \R^n$ be a compact set, and suppose that solutions to~\eqref{e:ode-perturb-orig} exist for all $x_0\in \mathcal C$. 
	Let $T^x(x_0)$, $T^{y_0}(x_0)$, and $T^{y}(x_0)$ be the time $t_{\max}$-flow map corresponding to this ODE for initial values $x(t)=y_0(t)=y(t)=x_0$.
	
	Then as $\ep\to 0$, the maps $T^x_t$ and $T^y_t$ are
	$O(\epsilon^2)$ uniformly close over $\mathcal{C}$ in $C^r$ topology, for all $t \in [0,t_{\max}]$. The constants in the $O(\cdot)$ depend on %Lipschitz constants of $g$ and 
	bounds on 
	$\max_{0\le k\le r+1, x_0\in \mathcal C} \ve{D^kT^{y_0}(x_0)}$
	(the first $r+1$ derivatives of the $y_0$-trajectories), and
	$\max_{0\le k\le r, x_0\in \mathcal C, 0\le t\le t_{\max}} \ve{D^kG(x,t)|_{x=y_0(t)}} $ (the first $r$ derivatives of $G$ on the $y_0$-trajectories).
\end{lemma}
\begin{proof}
    First, using \Cref{l:perturb_trajectory_bound}, we get that 
    \[ \norm{x - y_0}_{C^r} = O(\epsilon) \]
    Now, note that $T_t^y$ satisfies
    %\Snote{do we need $F$ to be linear here? -- proof below uses linearity}
    \begin{align*}
        \ddd{t} y(t)
        %& = F(y_0(t),t) + \epsilon F(y_1(t),t) + \epsilon G(y_0(t),t)\\
        & = F(y(t),t) + \epsilon G(y(t),t) + \epsilon(G(y_0(t),t) - G(y(t),t))\\
        & = F(y(t),t) + \epsilon G(y(t),t) + O(\epsilon^2)
    \end{align*}
    Now, by using \cref{l:perturb_trajectory_bound} again, we get that
    \[ \norm{x - y}_{C^r} = O(\epsilon^2) \]
    \Snote{We need to mention that the constants in O notation depend on the trajectory of $x$, and hence we need to get bounds on that, again using \cref{l:perturb_trajectory_bound}}
\end{proof}

\begin{corollary} %[\cite{turaev2002polynomial}]
	\label{l:perturbed_ode_cr}
	Consider the ODE
	\[ \dot{x} = Ax + \epsilon g(x,t) \]
	such that $\norm{A} = 1$ and $g$ has bounded $(r+1)^{th}$ derivatives on a compact set $\mathcal{C}$. Let $T^x$ be the flow map corresponding to this ODE. For fixed $x_0$, let $y_0, y_1$ be functions satisfying 
	\begin{align*} \dot{y_0} &= Ay_0 \\
	 \dot{y_1} &= Ay_1 + g(y_0(t),t) \end{align*}
	such that $y_0(0) = x_0$ and $y_1(0) = 0$. Consider the flow map $T^y : \R \times \R^n$ such that
	$T^y(t,x_0) = y_0(t) + \epsilon y_1(t)$. Then, the maps $T^x_t$ and $T^y_t$ are
	$O(\epsilon^2)$ uniformly close over $\mathcal{C}$ in $C^r$ topology, for all $t \in [0,2\pi]$. The constants in the $O(\cdot)$ depend on %Lipschitz constants of $g$ and 
	bounds on the first $r$ derivatives of the actual trajectories, and the first $r$ derivatives of $g$ on an open set containing the trajectories.
\end{corollary}
%\ifdefined\PROOF
\begin{proof}
	Since we are working in $C^2$ topology, we need to show that
	\[ \sup_{t \in [0,2\pi], x_0} \norm{T_t^x(x_0) - T_t^y(x_0)} + \norm{DT_t^x(x_0) - DT_t^y(x_0)} = O(\epsilon^2) \]
	First, we will show that
	\[ \sup_{t \in [0,2\pi], x_0} \norm{T_t^x(x_0) - T_t^y(x_0)} = O(\epsilon^2) \]
	Let $z(t) = T_t^x(x_0) - T_t^y(x_0)$, and let $w(t) = \norm{z_0}$. Then $w^2 = z^\intercal z$. Therefore,
	\begin{align*}
		\frac{d}{dt} (w^2) & = 2 z^\intercal \dot{z} \\
											 & = 2 z^\intercal \brac{Ax + \epsilon g(x,t) - Ay_0 - \epsilon Ay_1 - \epsilon g(y_0(t),t)} \\
											 & = 2 z^\intercal A z + 2 z^\intercal \epsilon \brac{g(x,t) - g(y_0,t)} \\
											 & \le 2 \norm{A} \norm{z}^2 + 2 \epsilon \norm{z} L_g \norm{x - y_0} \\
											 & = 2 \norm{A} \norm{z}^2 + 2 \epsilon \norm{z} L_g \norm{x - y + \epsilon y_1}\\
											 & \le \brac{2 \norm{A} + 2 \epsilon L_g} \norm{z}^2 + 2 \epsilon^2 L_g \norm{z} \norm{y_1}\\
											 \implies
		2 w \dot{w} & \le \brac{2 \norm{A} + 2 \epsilon L_g} w^2 + 2 \epsilon^2 L_g w \norm{y_1}\\
		\implies
		\dot{w} & \le \brac{\norm{A} + \epsilon L_g} w + 2 \epsilon^2 L_g \norm{y_1} 
	\end{align*}
	Let $\sup_{x_0,t} \norm{y_1} = M$, then using \Cref{l:linear_ode_upper_bound} with $a = \norm{A} + \epsilon L_g$ and $b = 2 \epsilon^2 L_g M$, we get an upper bound
	\[ w \le \epsilon^2 \brac{\frac{L_g M}{1 + \epsilon L_g} \brac{e^{2 \pi(1 + \epsilon L_g)} - 1}} = O(\epsilon^2) \]

	For the upper bound on $\norm{y_1}$, note that $\norm{y_1}$ satisfies
	\begin{align*}
		\frac{d}{dt} (\norm{y_1}^2)
	& = 2 y_1^\intercal A y_1 + 2 y_1^\intercal g(y_0,t) \\
	& \le 2 \norm{A} \norm{y_1}^2 + 2 \norm{y_1} M_g \\
	\implies
		\frac{d}{dt} (\norm{y_1}) & \le \norm{y_1} + M_g\\
		\implies
		\norm{y_1} & \le M_g \brac{e^{2 \pi} - 1}
	\end{align*}
	where $M_g = \sup_{x,t} = \norm{g(x,t)}$.

	\begin{equation}
		\label{eq:pertubation_bound}
		\norm{x - y} \le \epsilon^2 \brac{\frac{L_g M_g}{(1 + \epsilon L_g)} \brac{e^{2 \pi} - 1} \brac{e^{2\pi(1 + \epsilon L_g)} - 1}}
	\end{equation}

	Now, we will bound the derivatives, and show that
	\[ \sup_{t \in [0,2\pi], x_0} \norm{DT_t^x(x_0) - DT_t^y(x_0)} = O(\epsilon^2) \]
	Define $\alpha(t) = DT_t^x(x_0)$. then $\alpha(t)$ satisfies the ODE
	\begin{equation}
		\label{eq:x_derivative}
		\dot{\alpha} = A \alpha + \epsilon Dg(x(s),s) \alpha
	\end{equation}
	with the initial condition $\alpha(0) = \id$.
	This follows since 
	\[ T_t^x(x_0) = \int_0^t A T_s^x(x_0) + \epsilon g(T_s^x(x_0),s) ds \]
	We have
	\begin{align*}
		\alpha(t) = DT_t^x(x_0)
		& = \int_0^t D \brac{A T_s^x(x_0) + \epsilon g(T_s^x(x_0),s)} ds \\
		& = \int_0^t A DT_s^x(x_0) + \epsilon Dg(T_s^x(x_0),s) DT_s^x(x_0) ds \\
		& = \int_0^t A \alpha(s) + \epsilon Dg(x(s), s) \alpha(s) ds
	\end{align*}

	Let $T_t^{y_0}$ be the flow map of ODE $\dot{y_0} = A y_0$. Define $T_t^{y_1}(x_0) = y_1(t)$. Then we have
	\[ DT_t^{y}(x_0) = DT_t^{y_0}(x_0) + \epsilon DT_t^{y_1}(x_0) \]
	Now, define $\beta_0(t) = DT_t^{y_0}(x_0)$, and $\beta_1(t) = DT_t^{y_1}(x_0)$, and $\beta(t) = DT_t^{y}(x_0) = \beta_0(t) + \epsilon \beta_1(t)$. Then $\beta_0$ satisfies
	\begin{equation}
		\label{eq:y_0_derivative}
		\dot{\beta_0} = A \beta_0
	\end{equation}
	with initial condition $\beta_0(0) = \id$ 
	since
	\begin{align*}
		T_t^{y_0}(x_0)
		& = \int_0^t A T_s^{y_0}(x_0)ds\\
		\Rightarrow \beta_0(t) = DT_t^{y_0}(x_0)
		& = \int_0^t D \brac{A T_s^{y_0}(x_0)} ds \\
		& = \int_0^t A DT_s^{y_0}(x_0)ds \\
		& = \int_0^t A \beta_0(s) ds
	\end{align*}
	and $\beta_1$ satisfies
	\begin{equation}
		\label{eq:y_1_derivative}
		\dot{\beta_1} = A \beta_1 + Dg(y_0(s), s)\beta_0
	\end{equation}
	with initial condition $\beta_1(0) = 0$
	since
	\begin{align*}
		T_t^{y_1}(x_0) 
		& = \int_0^t A T_s^{y_1}(x_0) + g(T_s^{y_1}(x_0),s) ds\\
		\Rightarrow \beta_1(t) = DT_t^{y_1}(x_0)
		& = \int_0^t D \brac{A T_s^{y_1}(x_0) + g(T_s^{y_0}(x_0),s)} ds \\
		& = \int_0^t A DT_s^{y_1}(x_0) + Dg(T_s^{y_0}(x_0),s) DT_s^{y_0}(x_0) ds \\
		& = \int_0^t A \beta_1(s) + Dg(y_0(s), s) \beta_0(s) ds
	\end{align*}
	
	Let $v$ be a unit vector. Define $p = (\alpha - \beta)$, let $q = \norm{pv}$. Then $q^2 = v^\intercal p^\intercal p v$. Therefore,
	\begin{align*}
		\frac{d}{dt}(q^2)
		& = 2 v^\intercal p^\intercal \dot{p} v \\
		\Rightarrow q \dot{q} 
		& = v^\intercal p^\intercal (\dot(\alpha) - \dot(\beta)) v\\
		& = v^\intercal p^\intercal \brac{A \alpha + \epsilon Dg(x,t))\alpha - A \beta_0 - \epsilon A \beta_1 - \epsilon Dg(y_0,t) \beta_0} v \\
		& = v^\intercal p^\intercal \brac{Ap + \epsilon \brac{Dg(x,t)\alpha - Dg(y_0,t)\beta_0}} v\\
		& = v^\intercal p^\intercal A pv + \epsilon v^\intercal p^\intercal \brac{Dg(x,t) \alpha - Dg(x,t)\beta_0 + Dg(x,t)\beta_0 - Dg(y_0,t) \beta_0}v\\
		& = v^\intercal p^\intercal A pv + \epsilon v^\intercal p^\intercal \brac{Dg(x,t)(\alpha - \beta) + \epsilon Dg(x,t) \beta_1 + (Dg(x,t) - Dg(y_0,t)) \beta_0} v\\
		& \le \norm{A} q^2 + \epsilon \norm{Dg(x,t)} q^2 + \epsilon^2 \norm{pv} \norm{Dg(x,t)} \norm{\beta_1v} + \epsilon \norm{pv} \norm{x - y_0} \Lip(Dg) \norm{\beta_0 v}\\
		\Rightarrow \dot{q}
		& \le \brac{\norm{A} + \epsilon \Lip(g)} q + \epsilon^2 \Lip(g) \norm{\beta_1} + \epsilon (\norm{x - y} + \norm{\epsilon y_1}) \Lip(Dg) \norm{\beta_0}\\
		& \le \brac{\norm{A} + \epsilon \Lip(g)} q + \epsilon^2 (\Lip(g) \norm{\beta_1} + (\epsilon C_0 + \norm{y_1}) \Lip(Dg) \norm{\beta_0}) \labeleqn{eq:perturbation_derivative_ode}
	\end{align*}
	where $C_0$ is the constant from \eqref{eq:pertubation_bound}. Now, it suffices to bound $\norm{\beta_0}$ and $\norm{\beta_1}$.

	For any unit vector $v$, $\norm{\beta_0 v}$ satisfies
	\begin{align*}
		\frac{d}{dt} (\norm{\beta_0 v}^2)
		& = 2 v^\intercal \beta_0^\intercal A \beta_0 v\\
		\Rightarrow \frac{d}{dt} \norm{\beta_0 v}
		& \le \norm{A} \norm{\beta_0 v}
	\end{align*}
	therefore, by \Cref{l:linear_ode_upper_bound}, $\norm{\beta_0} \le \sup_v \norm{\beta_0 v} \le \norm{\beta_0(0)} e^{2 \pi} = e^{2 \pi}$ since $\norm{A} = 1$ and $\norm{\beta_0(0)} = 1$. Similarly, for any unit vector $v$, $\norm{\beta_1v}$ satisfies
	\begin{align*}
		\frac{d}{dt} (\norm{\beta_1 v}^2)
		& = 2 v^\intercal \beta_1^\intercal (A \beta_1 + Dg(y_0,t) \beta_0) v\\
		\Rightarrow \frac{d}{dt} \norm{\beta_1 v}
		& \le \norm{A} \norm{\beta_1 v} + \norm{Dg(y_0,t)} \norm{\beta_0v}\\
		& = \norm{A} \norm{\beta_1 v} + \Lip(g) e^{2\pi} 
	\end{align*}
	therefore, by \Cref{l:linear_ode_upper_bound}, $\norm{\beta_1} \le (\Lip(g) e^{2\pi}) (e^{2\pi} - 1)$, since $\norm{A} = 1$ and $\norm{\beta_1(0)} = 0$.
	Substituting everything back into \eqref{eq:perturbation_derivative_ode}, and applying \Cref{l:linear_ode_upper_bound}, we get
	\begin{equation}
		\label{eq:perturbation_derivative_bound}
		\norm{DT_t^x(x_0) - DT_t^y(x_0)} \le \epsilon^2 \brac{\frac{\Lip(g)^2 e^{2\pi}(e^{2\pi} - 1) + (\epsilon C_0 + M_g (e^{2\pi} - 1)) \Lip(Dg) e^{2 \pi}}{1  + \epsilon \Lip(g)}} \brac{e^{2\pi (1 + \epsilon \Lip(g))}} 
	\end{equation}
	Thus, we prove the required result.
\end{proof}
%\fi

\begin{lemma}
\label{l:perturb_trajectory_bound}
    Consider the ODE
    \begin{align}\label{e:ode-perturb-exist}
        \ddd t x(t) &= F(x(t),t) + \ep G(x(t),t)
    \end{align}
    where $x:[0,t_{\max}]\to \R^n$, $F,G:\R^n\times \R\to \R$, and 
    $F(x,t)$, $G(x,t)$ are $C^1$. Let $\mathcal C$ be a compact set, and suppose that for all $x_0\in \mathcal C$, solutions to~\eqref{e:ode-perturb-exist} with $x(0)=x_0$ exist for $0\le t\le t_{\max}$ and $\ep=0$.
    Then there exists $\ep_0$ such that solutions to~\eqref{e:ode-perturb-exist} with $x(0)=x_0$ exist for $0\le t\le t_{\max}$ and $0\le \ep<\ep_0$.
    
    Moreover, letting $x^{(\ep)}(t)$ be the solution with given $\ep$, we have that as $\ep\to 0$, $\ve{x^{(\ep)}(t)-x^{(0)}(t)}=O(\ep)$, where the constants in the $O(\cdot)$ depend only on $\max_{0\le t\le t_{\max}, x_0\in \mathcal C}\ve{DF(x^{(0)}(t),t)}$ (the Lipschitz constant of the $\ep=0$ trajectories) and $\max_{0\le t\le t_{\max}, x_0\in \mathcal C} \ve{G(x^{(0)}(t),t)}$ (the maximum of $G$ on the $\ep=0$ trajectories).
\end{lemma}
\begin{proof}
    \Snote{add proof of existence of $\epsilon_0$}
    
    Let $F_{\epsilon}(x,t) = F(x,t) + \epsilon G(x,t)$, and let $T_t^\epsilon(x_0)$ denote the flow map of~\eqref{e:ode-perturb-exist} starting at $x_0$.
    From~\eqref{l:Dr}, we get that 
    \begin{equation}
        \ddd{t} \partial_{i_1 \cdots i_r} T_t^{\epsilon}(x_0) = \sum_{i=1}^d \partial_i F_\epsilon(x^{(\epsilon)},t) \partial_{i_1 \cdots i_r} T_{t,i}^\epsilon + G(DF_\epsilon, \ldots, D^r F_\epsilon, DT_t^\epsilon, \ldots, D^{r-1} T_t^\epsilon)    
    \end{equation}
    Plugging in $\epsilon = 0$ in the equation above, we get
    \begin{equation*}
        \ddd{t} \partial_{i_1 \cdots i_r} T_t^{0}(x_0) = \sum_{i=1}^d \partial_i F(x^{(0)},t) \partial_{i_1 \cdots i_r} T_{t,i}^{y_0} + G(DF, \ldots, D^r F, DT_t^{0}, \ldots, D^{r-1} T_t^{0})
    \end{equation*}
    We will now show that these two trajectories are $O(\epsilon)$ uniformly close using induction. \fixme{missing the base step}.
    
    By induction hypothesis, we know that for all $k < r$, $\norm{D^k T_t^\epsilon - D^k T_t^0} = O(\epsilon)$. Further, observe that $\norm{T_t^\epsilon(x_0) - T_t^0(x_0)} = O(\epsilon)$, and $D^k F_\epsilon - D^k F = \epsilon D^k G = O(\epsilon)$ (this holds for $k \le r$), which implies that
    \begin{align*}
       \norm{D^k F_\epsilon(x^{(\epsilon)},t) - D^k F(x^{(0)},t)}
       & \le \norm{D^k F_\epsilon(x^{(\epsilon)},t) - D^k F(x^{(\epsilon)},t)} + \norm{D^k F(x^{(\epsilon)},t) - D^k F(x^{(0)},t)}\\
       & \le \epsilon \norm{G(x^{(\epsilon)},t)} + \norm{x^{(\epsilon)} - x^{(0)}} \norm{D^k F(x,t)} 
    \end{align*}
    Therefore, $\norm{D^k F_\epsilon(x^{(\epsilon)},t) - D^k F(x^{(0)},t)} = O(\epsilon)$, where constants in $O(\cdot)$ depend on $\norm{x^{(0)} - x^{(\epsilon)}}$, and $\norm{D^k F(x^{(0)},t)}$. \Snote{The evaluation point can be anywhere between $x^{(0)}$ and $x^{(\epsilon)}$ right?} \hlnote{Not a big deal---when we take $\ep\to 0$, $x^{(\ep)}\to x^{(0)}$ so the max approaches the max on the trajectory}
    Since $G$ is a fixed polynomial that depends on $i_1, \ldots, i_r$, this gives the bound
    \[ \norm{G(DF_\epsilon, \ldots, D^r F_\epsilon, DT_t^{\epsilon}, \ldots, D^{r-1} T_t^{\epsilon}) - G(DF, \ldots, D^r F, DT_t^{0}, \ldots, D^{r-1} T_t^{0})} = O(\epsilon) \]
    Therefore, we get
    \begin{align*}
        \ddd{t} \partial_{i_1 \cdots i_r}(T_t^\epsilon - T_t^0)
        & = \sum_{i=1}^d \partial_i F_\epsilon(x^{(\epsilon)}, t) \partial_{i_1 \cdots i_r} T_{t,i}^\epsilon - \sum_{i=1}^d \partial_i F(x^{(0)}, t) \partial_{i_1 \cdots i_r} T_{t,i}^0 + O(\epsilon)\\
        & \le \sum_{i=1}^d \partial_i F(x^{(0)}, t) \partial_{i_1 \cdots i_r} (T_{t,i}^\epsilon - T_{t,i}^0) + \sum_{i=1}^d (\partial_i F_\epsilon(x^{(\epsilon)}, t) - \partial_i F(x^{(0)},t)) \partial_{i_1 \cdots i_r} T_{t,i}^\epsilon + O(\epsilon) \\
        & \le DF(x^{(0)},t) \partial (T_t^\epsilon - T_t^0) + O(\epsilon) 
    \end{align*}
    \Snote{might need to convert everything to norms to apply Gronwall}
    Now, a Gr\"onwall arguement gives us the bound,
    \[ \norm{\partial_{i_1 \cdots i_r} (T_t^\epsilon - T_t^0)} \le e^{t_{\max}} O(\epsilon) \]
\end{proof}


\subsection{Gr\"onwall lemma}

The following lemma is very useful for bounding the growth of solutions, or errors from perturbations to ODE's.

\begin{lemma}[Gr\"onwall]\label{l:gronwall}
    If $x(t)$ is differentiable on $t\in [0,t_{\max}]$ and satisfies the differential inequality
    \begin{align*}
        \ddd t x(t) &\le ax(t) + b,
    \end{align*}
    then 
    \begin{align*}
        x(t) &\le (bt+x(0)) e^{at}
    \end{align*}
    for all $t\in [0, t_{\max}]$.
\end{lemma}
